Pre-train or Annotate? Domain Adaptation with a Constrained Budget

Recent work has demonstrated that pre-training in-domain language models can boost performance when adapting to a new domain. However, the costs associated with pre-training raise an important question: given a fixed budget, what steps should an NLP practitioner take to maximize performance? In this paper, we view domain adaptation with a constrained budget as a consumer choice problem, where the goal is to select an optimal combination of data annotation and pre-training. We measure annotation costs of three procedural text datasets, along with the pre-training costs of several in-domain language models. The utility of different combinations of pre-training and data annotation are evaluated under varying budget constraints to assess which combination strategy works best. We find that for small budgets, spending all funds on annotation leads to the best performance; once the budget becomes large enough, however, a combination of data annotation and in-domain pre-training yields better performance. Our experiments suggest task-specific data annotation should be part of an economical strategy when adapting an NLP model to a new domain.

==> sections/8_related.tex <==
A number of recent studies have explored current and potential future negative externalities associated with the recent trend towards large-scale pre-training in NLP.  These include the carbon emissions generated by training models with larger and larger computational costs \citep{Strubell2019EnergyAP, schwartz2019green}, and the increased barriers to entry created by reliance on specialized hardware \citep{bender2021dangers}.  This line of work has called on the NLP community to evaluate not only a method's accuracy on held-out test data but also the amount of computation that is required during learning and inference.  

%\begin{itemize}
%    \item Green AI \citep{schwartz2019green, Strubell2019EnergyAP, patterson2021carbon}
%\end{itemize}

==> sections_old/0_abstract.tex <==

% Pre-trained language model-based domain adaptation has received much attention nowadays due to the success of BERT \citep{Devlin2019BERTPO}. Even though many proposed methods have been tested respectively to be beneficial, how they compare with each other remains unclear, which makes it hard for people to approach a new domain realistically. In this work, we present an empirical study into PLM-based DA techniques in the context of procedural text understanding, where we compare different approaches across multiple frameworks fairly to give insights in method selection. \FB{The second and third sentences are duplicate.} We first compare two popular pre-training-based unsupervised DA methods \FB{It is not clear what these two methods are}, and find that pre-training a language model on in-domain corpus from scratch leads to a better domain-specific PLM compared to fine-tuning the off-the-shelf PLM, demonstrating the importance of the customized vocabulary. Moreover, we show that simply annotating more labeled data for training is more helpful than pre-training in the low-resource setting given the same budget. Finally, we reveal that supervised DA approach may not perform as well as the pre-training-based approach but these two frameworks can work together to improve the target task performance. 

% Pre-trained language model-based domain adaptation has received much attention nowadays due to the success of BERT \citep{Devlin2019BERTPO}. 
% Domain-specific pre-training has received much attention nowadays due to its usefulness \citep{Gururangan2020DontSP}.
% However, those pre-training-based approaches might not be easily applied in a practical setting as they are prohibitive cost-wise \citep{Strubell2019EnergyAP}.
% However, practically those pre-training-based approaches are less applicable as their cost is prohibitive \citep{Strubell2019EnergyAP}.
% \FB{This sentence can be improved.}
% Therefore, one natural question is, given the limited budget, should we do domain-specific pre-training or even simply annotating more training data of the target task when approaching a new domain?
% Despite their usefulness, one practical issue of domain-specific pre-training approaches is their prohibitive cost. 
% Pre-training-based domain adaptation approaches have shown great performance with or without labeled data in a target domain.
% However, one practical issue of those approaches is their prohibitive computational cost.
Pre-training-based domain adaptation approaches now prevail as they can effectively adapt to a target domain by masked language modeling on unlabeled text. 
% However, one practical issue of those approaches is their prohibitive computational cost.
However, given their prohibitive computational cost, could it be more beneficial to use supervised domain adaptation methods under the same budget? 
% We are specifically interested in the scenario in which no target domain labeled data is available in the beginning, and a limited budget is given, we want to the result of the target domain task to be as good as possible. 
In this paper, we are interested in the scenario where our target domain is different from both the labeled and pre-training text, and we want to use a limited budget to boost our performance as much as possible.
% \citep{Gururangan2020DontSP, Strubell2019EnergyAP}. 
% Given a limited budget, a natural question when approaching a new domain is whether we should prioritize domain-specific pre-training or more training data annotation of the target task.
% When approaching a new domain with a limited budget, a common question is whether we should prioritize data-driven unsupervised methods like in-domain pre-training or supervised methods like task-specific data annotation.
% In this paper, we study domain-specific pre-training from a practical standpoint with regards to procedural text understanding in two parts. 
% In this paper, we study the applicability of domain adaptation methods from a practical standpoint with regards to procedural text understanding in two parts.
% In this paper, we compare the applicability of these two types of methods with regards to procedural text understanding.
To address this scenario, we explore both pre-training-based and supervised domain adaptation methods in the domain of procedural text understanding considering not only their performance but also their cost.
% where we not only experiment with different unsupervised pre-training approaches but also compare them with supervised methods in a budget-aware setting.
% In the first part, we explore different in-domain pre-training strategies.
% We first explore different data-driven unsupervised domain adaptation techniques.
% We try two popular methods on our collected procedural corpus: pre-training a language model from scratch and fine-tuning the off-the-shelf language model.
% To facilitate the comparison, we first explored unsupervised domain adaptation by experimenting with two popular pre-traning methods on our collected procedural corpus: 1) pre-training an in-domain language model from scratch; 2) fine-tuning the off-the-shelf language model.
We first experiment with two popular pre-traning methods on our collected procedural corpus: 1) pre-training a language model from scratch; 2) fine-tuning an off-the-shelf language model.
% Our finding is that pre-training from scratch leads to a better domain-specific language model, possibly because it uses a customized vocabulary and much more computation.
Our finding is that pre-training from scratch leads to a better performing domain-specific language model possibly because it uses a customized vocabulary and consumes much more computation.
% compared to fine-tuning the off-the-shelf language model.
% Our two findings are: 1) Pre-training from scratch leads to a better domain-specific language model \FB{Need reason}; 2) Increasing the size of the pre-training corpus while maintaining the proportion of procedural text can further improve the downstream task performance \FB{Remove this}.
% Moreover, we demonstrate that, under the same budget, simply annotating more training data for the downstream tasks is more helpful than the pre-training approach in the low-resource scenario. 
% Finally, we reveal that the supervised domain adaptation approach can even outperform the pre-training-based approach for some tasks, and these two types of methods can work together to further improve the target task performance.
% In the second part, we investigate how to use labeled data to boost target domain tasks. 
% In the second part, we investigate the applicability of the pre-training approach by comparing it with the supervised domain adaptation method.
% Then we investigated supervised domain adaptation methods and compared them with unsupervised pre-training methods in a realistic setting.
% Then we investigated the supervised domain adaptation framework \textsc{EasyAdapt} and revealed that it can perform on par with the pre-training methods on some tasks, signalling an effective and cost-friendly alternative.
Then we compare the two above methods with two supervised methods: 1) task-specific annotation; 2) \textsc{EasyAdapt}, in the budget-aware setting.
% We demonstrate that annotating more in-domain training data should be the priority when approaching a new domain as it results in a larger performance gain than the pre-training approach under a lower budget.
% We revealed that the supervised domain adaptation framework \textsc{EasyAdapt} can perform on par with the data-driven unsupervised methods on some tasks, signalling an effective and cost-friendly alternative.
% Moreover, we reveal that the supervised domain adaptation framework \textsc{EasyAdapt} can further boost the downstream task performance on top of the domain-specific pre-trained language model. 
% Moreover, in a budget-aware comparison, we showed that supervised domain adaptation should be the priority as it results in a larger performance gain under a lower budget while the unsupervised pre-training approaches are more effective with a higher budget.
% Moreover, in a budget-aware comparison, we showed that supervised domain adaptation results in a larger performance gain, making it preferable to the unsupervised pre-training approaches under a lower budget.
% Finally, in the budget-aware comparison, we showed that \textsc{EasyAdapt} and task-specific annotation result in a larger performance gain, making it preferable to the pre-training approaches under a lower budget.
We reveal that supervised methods can result in a larger performance gain under a lower budget, especially for \textsc{EasyAdapt}, which utilizes out-of-domain data to help the target domain task. 
As the budget increases, the benefit from labeled data diminishes, and the pre-training methods start to stand out making it more preferable to supervised methods in high-resource scenario.
% With the incorporation of \textsc{EasyAdapt} into the domain-agnostic language model, it can perform on par with the in-domain language model on some tasks, signalling an effective and cost-friendly alternative.

% : unsupervised domain-adaptive pre-training, more labeled data in the target domain and supervised domain adaptation, . 


% Even though many proposed methods have been tested respectively to be beneficial, how they compare with each other remains unclear. \FB{The abstract is still not clear enough for example what "methods" are proposed, so maybe we can start with the "Don't stop pre-training paper" as the background introduction.}
% In this work, we present an empirical study on how to approach a new domain with the pre-tarined language model from three directions: unsupervised domain-adaptive pre-training, more labeled data in the target domain and supervised domain adaptation, in the context of procedural text understanding. 
% We first compare two popular pre-training-based methods, pre-training a language model from scratch and in-domain fine-tuning the off-the-shelf language model.
% We find that pre-training from scratch leads to a better domain-specific language model.
% Then we show that increasing the size of the pre-training corpus by adding non-procedural text (from the same areas) can also bring in some decent performance boost. \FB{Be specific here.}
% Moreover, we demonstrate that, given the same budget, simply annotating more training data for the downstream tasks is more helpful than the pre-training approach in the low-resource setting. Finally, we reveal that the supervised domain adaptation approach can even outperform the pre-training-based approach for some tasks, and these two types of methods can work together to improve the target task performance. 



==> sections_old/1_intro.tex <==
\begin{figure}[h]
\includegraphics[width=\columnwidth]{figures/budget-crop.pdf}
\caption{\label{fig:consumer_choice} We view domain adaptation as a consumer choice problem.}
\end{figure}

Natural Language Processing practitioners are often faced with a situation where they need to apply an existing system to texts from a new domain or genre that substantially differ in style or topic from the corpus the system was developed for.  Current NLP methods perform poorly in this situation, so prior research on domain adaptation has investigated both supervised and unsupervised methods.  Semi-supervised learning \citep{blum1998combining,xie2019unsupervised} and unsupervised domain adaptation \citep{blitzer2006domain,ganin2015unsupervised,ruder2018strong} offer a set of methods that improve classification performance by training on large quantities of unlabeled data in conjunction with out-of-domain supervised data.  Much prior literature in this area has claimed obtaining labeled data is expensive, or that it is simply not available, without empirically comparing the costs associated with annotating in-domain data against the costs of training on large quantities of unsupervised datasets.

More recent work has shown that pre-training transformers using a masked language model objective on unlabeled data in the target domain is an effective method for both unsupervised domain adaptation \cite{Han2019UnsupervisedDA} and also boosts performance when in-domain annotations are available \cite{Gururangan2020DontSP}.  Despite recent advances in domain adaptation and domain-adaptive pretraining, the question remains: given a fixed budget for improving performance on a target domain, what steps should an NLP practitioner take?  One the one hand they could simply choose to hire annotators to label in-domain data, while on the other hand they could rent GPUs or TPUs to pre-train large language models on (unlabeled) in-domain data.  This raises an important question - given a fixed budget for adapting to a new domain, is it better to spend your money pretraining on large, unlabeled in-domain corpora, annotating supervised data in the target domain, or a combination of the two?


%We analyze the tradeoffs between annotation and pretraining using adaptation to several new procedural text genres and domains as a case study.  We empirically measure the cost of annotating in-domain data, and also the cost of in-domain pretraining.

In this paper we view the NLP practitioner’s dilemma of how to adapt to a new domain as a problem of consumer choice, a classic problem in microeconomics \citep{becker1965theory,lancaster1966new}.  
As illustrated in Figure \ref{fig:consumer_choice}, the NLP practitioner (consumer) can purchase $X_a$ annotated documents (by hiring annotators) at a cost of $C_a$ each, and $X_p$ pretraining epochs (by renting GPUs or TPUs) at a cost of $C_p$.  Given a fixed budget, $B$, the consumer can choose any combination that fits within the budget constraint $X_a C_a + X_p C_P \leq B$.  The problem faced by the consumer is then to choose an optimal combination of annotation and pre-training to maximize a utility function within a fixed budget.  The utility function, $U(X_a, X_p)$ is based on an appropriate performance metric, for example, $F_1$ score, measured after pretraining for $X_p$ epochs and then fine-tuning on $X_a$ annotated in-domain documents.

To empirically measure $C_a$, the cost of annotation, we hired in-house annotators to manually label in-domain documents for supervised fine-tuning in 3 procedural text domains (wet-lab protocols, experimental paragraphs extracted from journal articles, and chemical synthesis procedures described in patents). We also measured the costs of in-domain pretraining, $C_p$, on a large collection of unlabeled procedural texts using Google's cloud TPUs.
The utility of different combinations of pretraining, and annotation, $U(X_a, X_p)$, is then empirically evaluated using varying budget constraints in ${3 \choose 2} = 6$  (source $\rightarrow$ target) combinations in \S \ref{sec:label}.

For small budgets, we find that in-domain annotation is a clearly superior strategy, however, as more funds become available, a combination of pretraining and annotation appears to be the best choice.  
%Although our analysis is limited to 3 procedural text domains, where we have experimental data available on the costs of annotation, or ${3 \choose 2} = 6$ (source $\rightarrow$ target) combinations, 
Our results suggest that given current costs of pre-training large transformer models such as BERT \citep{Devlin2019BERTPO} and RoBERTa \citep{Liu2019RoBERTaAR}, in-domain data annotation should always be part of an economical strategy when adapting an NLP model to a new domain.



\begin{comment}

% Assume we have labeled data in multiple domains (including the target), a large unlabelled corpus in the target domain and a domain-agnostic pre-trained language model, we want to compare three useful strategies, i.e., in-domain pre-training, annotating more data in the target domain and utilizing out-of-domain labeled data via supervised DA techniques, from different perspectives (such as performance improvement and cost) to see which one is the best option.

% BERT \citep{devlin-etal-2019-bert}, a transformer-based language model pre-trained on a large amount of unlabelled corpus, has received much attention nowadays as it can lead to remarkable performance gain on various NLP tasks. 

As demonstrated through BERT \citep{Devlin2019BERTPO} and its variants \citep{Liu2019RoBERTaAR, Sanh2019DistilBERTAD}, pre-training a language model on a large amount of unlabelled corpus has been proven to be a robust and generalizable technique, which can lead to remarkable performance gain on various NLP tasks. Therefore, it is also widely studied and used in the field of domain adaptation. \FB{Cost benefit trade-off}

Among all pre-trained language model-related domain adaptation research, one prevailing direction is to build a domain-specific language model in an unsupervised manner because the language model pre-trained on general English corpus turns out to be less effective when applied to tasks from specific domains, like bio-medicine and social media. The main reason of this performance degradation that there is a language distribution mismatch between the pre-training corpus and the tackled downstream tasks. To bridge this "domain" gap, many pre-training-based methods have been proposed. For instance, \citet{Beltagy2019SciBERTAP} pre-trains a language model from scratch on the collected scientific literature corpus, which produces great results on scientific tasks. Moreover, \citet{Gururangan2020DontSP} demonstrates that continuing pre-training the off-the-shelf pre-trained language model on in-domain corpus can also address the problem of domain mismatch. However, there is no conclusion about which method works better as those methods have not been compared on the same dataset. More importantly, pre-training-based approaches
% require a huge amount of unlabeled text, which may not be available or hard to collect because of the ethical concerns for some of the domains. Also they
are computationally demanding and thus prohibitive cost-wise \citep{Strubell2019EnergyAP}. Directly using pre-training-based approaches may not be the optimal solution especially in low-resource scenarios. However, a better solution could be increasing labeled training data to obtain a larger performance boost \citep{Garrette2013LearningAP}.

Another popular trend for pre-trained language model-related domain adaptation methods is to use the pre-trained language model as the representation learner and incorporate it into traditional domain adaptation frameworks such as Feature Augmentation (FA) \citep{Li2020SemisupervisedDA} and Mixture of Experts (MoE) \citep{Wright2020TransformerBM}, which can take advantage of out-of-domain labeled data. Although traditional domain adaptation frameworks can benefit from the generated contextual embedding, it is not clear how the performance gains they get compare with the gains obtained from unsupervised pre-training-based approaches, and how they can work together to further improve the performance. 

% Therefore, what is lacking is a realistic comparison between different pre-trained language model-based domain adaptation methods, which can give insight and help people to find the best practical solution to approach a new domain. In light of this, we present an empirical study into PLM-based DA techniques, where we not only compare different approaches within the same framework but also compare different frameworks \FB{It is not clear what the difference between "approach" and "framework" is.} and explore how the performance of models changes under varying setups so that we can access the trade-off in method selection from the practical perspective. 

Therefore, what is lacking is a realistic comparison between different domain adaptation methods, which can give insight on finding the best practical solution to approach a new domain. In light of this, we present an empirical study on three feasible directions: 1) domain-specific pre-training; 2) more target domain training data; 3) supervised domain adaptation. We compare these three directions from multiple perspectives such as performance and cost, and explore how the performance of those methods changes under varying setups to access the trade-off in method selection.


This paper consists of two parts. In the first part, we focus on comparing two prominent pre-training-base techniques previously mentioned. \FB{Past tense starting from here.}
% , pre-training a language model from scratch and in-domain fine-tuning the off-the-shelf pre-trained language model, 
We experiment two methods on the domain of procedural text, which is a special genre of text instructing how a specific task is carried out. We collect a large procedural text corpus from three different sources (PubMed articles, chemical patents and cooking recipes) containing around 1.1 billion words for pre-training, and then compare two above strategies on 6 related datasets including two self-built ones. The empirical results show that pre-training from scratch with the customized vocabulary brings a better domain-specific PLM, and increasing the size of pre-training corpus can help improve the downstream tasks performance.

\FB{Past tense.} In the second part, we studied how to use the labeled data with the pre-training a language model efficiently to relieve the domain shift. As the pre-training approach is costly, we first explore whether simply adding more labeled target domain training data is more effective than the pre-training given the same budget. It turns out that the pre-training approach is more effective when there is a relatively large training set.
% with the simple method of annotating more  to investigate the feasibility and necessity of each method realistically. 
Then we investigated the pre-trained language model-based supervised domain adaptation method. Utilizing the labeled data from other domains, we saw how it compares to the data-driven unsupervised approaches and tried different configurations to find the best way to integrate both types of methods. As a result, we find that although supervised domain adaptation method can outperform in-domain pre-training method on some tasks, fusing two frameworks leads to a better performance especially when each domain has its own language model for feature generation.

In summary, we make the following contributions:

(1) We compared different pre-training-based domain adaptation methods in the context of procedural text understanding, and showed that pre-training from scratch with the in-domain vocabulary works the best.

(2) We presented ProcBERT, a procedural corpus-pretrained language model, which outperforms competitive baselines like SciBERT and BioMed-RoBERTa on a range of related datasets. 
% \FB{I guess maybe we can talk about the comparison (in-domain pre-training V.S. labelling more data in the second contribution.)}

(3) We conducted careful analysis to explore the effectiveness and necessity of the in-domain pre-training given budget constraints, and concluded that pre-training approach should be considered only if the size of training data of downstream tasks is relatively large.

(4) We compared the supervised domain adaptation approach with the pre-training approach, and found that supervised domain adaptation approach can perform better on some tasks and these two lines of methods can be incorporated to further boost the performance on the target tasks.

\end{comment}

==> sections_old/2_pretrain.tex <==


% In this section, we compare procedural text-related LMs pre-trained with different strategies and also other off-the-shelf PLMs in terms of performance.

% The focus of this section is to compare the in-domain pre-training techniques (unsupervised methods) in the context of procedural text understanding.

% In this section, we research domain-specific pre-training in the context of procedural text understanding. 
% We first collect a billion-level procedural text corpus and then experiment with two state-of-the-art in-domain pre-training methods to build a state-of-the-art procedural-text-specific pre-trained language model.
% Pre-training-based unsupervised domain adaptation has recently drawn much attention because it can mitigate the domain mismatch between a pre-training corpus and a tackled task with an unlabeled target domain corpus.
% This occurs regardless of whether the labeled data is from the source domain \citep{Han2019UnsupervisedDA} or the target domain \citep{Gururangan2020DontSP} in the later fine-tuning stage.
% However, one non-negligible downside is its prohibitive computational cost \citep{Strubell2019EnergyAP}, which makes it less applicable in practice. To enable the research on the applicability of pre-training-based domain adaptation, in this section, we experiment with two state-of-the-art unsupervised pre-training methods on our collected corpus in the domain of procedural text understanding.
To enable the comparison of different domain adaptation methods under the cost-aware setting, in this section we first explore two pre-tarining-based domain adaptation methods on procedural text understanding. We start with the collection of pre-training procedural corpus in \S\ref{sec:corpus_collect}. Then in \S\ref{sec:pre-training} we lay out the details of two pre-training methods, model configuration and implementation choices. We close by showing the performance of two pre-trained models on selected downstream datasets (\S\ref{sec:downstream}).

% We experiment with two methods, pre-training a domain-specific language model from scratch and continuing pre-training the domain-agnostic language model on in-domain corpus, on our collected corpus to build procedural-text-specific pre-trained language models in the following section. 

% In this section, we compare two pre-training-based DA methods in the context of procedural text understanding, i.e., pre-training a domain-specific language model from scratch and continuing pre-training the domain-agnostic language model on in-domain corpus. \FB{I need to change the story here as we only experiment the fine-tuning method on the smaller dataset.} For the first method, we use the configuration \texttt{BERT-base} denoted as \textsc{ProcBERT}. For the second method, we continue pre-training \textsc{RoBERTa} on procedural text following \citep{Gururangan2020DontSP} denoted as \textsc{Proc-RoBERTa} \FB{The model names should be on the same page.}.

% \subsection{Tokenization \& Vocabulary}

\subsection{Corpus Collection}
\label{sec:corpus_collect}
The first step to pre-train a language model is to get a large amount of unlabelled corpus. Unlike other language models using existing corpus such as Wikipedia \citep{Zhu2015AligningBA} and CommonCrawl \citep{Negal2016CC} for pre-training, the procedural corpus needs to be collected from scratch as there is no such corpus available, and it is hard to collect for two reasons: 1) Procedural text is often mixed with other text, e.g., experimental procedures are usually described in the scientific papers, but they only take a few paragraphs; 2) There are procedural text from different domains, such as lab biochemistry protocols and cooking recipes. 
Therefore, we selected three sources to collect procedural corpus: PubMed articles, chemical patents and recipes, to get relatively large amount of data and at the same time cover as many domains as we can. 
For PubMed articles, we first trained a procedural paragraph extractor by fine-tuning SciBERT \citep{Beltagy2019SciBERTAP} on the SciSeg dataset \citep{Dasigi2017ExperimentSI}, and then applied the trained extractor to the {\em Materials and Methods} section of PubMed articles to obtain procedural paragraphs. Similarly, for chemical patents, we applied the reaction extractor developed by \citet{Lowe2012ExtractionOC}, which is a trained Naive Bayes classifier, to the {\em Description} section of all our patent corpus.  
More details of extracting procedural paragraphs from PubMed articles and chemical patents can be found in Appendix \ref{sec:app_corpus}. For recipes, we directly use the text component of Recipe1M+ dataset \citep{Marn2019Recipe1MAD} as it is the largest recipe dataset publicly available.
% For PubMed articles and chemical patents, we first trained a procedural paragraph extractor using the existing dataset from the {\em Materials and Methods} section and the {\em Description} section respectively. More details of extracting procedural paragraphs from PubMed articles and chemical patents can be found in Appendix \ref{sec:corpus}. For recipes, we directly use the text component of Recipe1M+ dataset \citep{Marn2019Recipe1MAD} as it is the largest recipe dataset publicly available.
As a result, our collected corpus \textsc{Procedure} includes around 1.1 billion words in total, and we show its statistics together with the statistics of other corpora used in the language model pre-training in Table \ref{tab:corpus_size}. 
Clearly, the size of our corpus is far smaller compared to other corpora, so we created an extended version \textsc{Procedure+}, where we up-sampled the procedural paragraphs 6 times and combined them with the original full text of PubMed articles and chemical patents to make sure at least half of data is procedural text, leading to a larger corpus containing around 12 billion words. 


% \begin{table}[t!]
% \small
% \begin{center}
% % \setlength\tabcolsep{3pt}
% \begin{tabular}{ccc}
% \hline Model & Corpus & \# Tokens / Text Size  \\ \hline
% BERT & Wiki + Books & 3.3B / 16GB \\ 
% RoBERTa &  Web crawl & - / 160GB \\
% SciBERT & PMC + CS &  3.2B / - \\ 
% BioMed-RoBERTa & BioMed & 7.6B / 47GB \\ \hline
% Procedure (extract)  & all & 1.1B / 6.5GB  \\ 
%   & PubMed &   \\ 
%   & Chem. patent &   \\ 
%   & Recipe &   \\ \hline
% Procedure (full)  &  & 12B / 77GB  \\ 
% %  & PubMed & 0.32B &  \\ 
% %  & Chem. Patent & 0.62B & - \\ 
% %  & Recipe & 0.12B & - \\ \hline
% % ProcBERT (full) & - & 12.4B words \\
% \hline
% \end{tabular}
% \end{center}
% \caption{\label{tab:corpus_size} A summary of statistics for pre-training corpus.}
% \end{table}


\begin{table}[t!]
\small
\begin{center}
% \setlength\tabcolsep{3pt}
\scalebox{0.85}{
\begin{tabular}{lccc}
% \hline Corpus & \# Tokens / Text Size & Model  \\ \hline
% Wiki + Books & 3.3B / 16GB & BERT \\ 
% Web crawl & - / 160GB & RoBERTa  \\
% PMC + CS &  3.2B / - & SciBERT \\ 
% BioMed & 7.6B / 47GB & BioMed-RoBERTa  \\ \hline
% Procedure  & 1.05B / 6.5GB  \\ 
% \indent - PubMed & 0.32B / 2.0GB  \\ 
% \indent - Chem. patent & 0.61B / 3.9GB \\ 
% \indent - Recipe & 0.11B / 0.6GB  \\ \hline
% Procedure^+  & 12B / 77GB  \\ 
\hline Corpus & \# Tokens & Text Size & Model  \\ \hline
Wiki + Books & 3.3B & 16GB & BERT \\ 
Web crawl & - & 160GB & RoBERTa  \\
PMC + CS &  3.2B & - & SciBERT \\ 
BioMed & 7.6B & 47GB & BioMed-RoBERTa  \\ \hline
\textsc{Procedure}  & 1.05B & 6.5GB & -  \\ 
\hspace{1mm} - PubMed & 0.32B & 2.0GB & -  \\ 
\hspace{1mm} - Chem. patent & 0.61B & 3.9GB & - \\ 
\hspace{1mm} - Recipe & 0.11B & 0.6GB & -  \\ \hline
\textsc{Procedure+}  & 12B & 77GB & -  \\ 
\hspace{1mm} - Procedural text & 6.3B & 39GB & - \\ 
\hspace{1mm} - Full articles & 5.7B & 38GB & - \\ 
\hline
\end{tabular}
}
\end{center}
\caption{\label{tab:corpus_size} The statistics of the pre-training corpora.}
\end{table}

\subsection{Pre-training Process}
\label{sec:pre-training}
% In this section, we outline the details of pre-training two procedural-text-specific language models: 
In this section, we outline the details of pre-training two procedural-text-specific language models with two different strategies:
1) \textsc{ProcBERT}, a language model pre-trained from scratch using our collected procedural corpus (\S\ref{sec:corpus_collect}) ; 2) \textsc{Proc-RoBERTa}, an in-domain fine-tuned \textsc{RoBERTa}-based language model. 

\subsubsection{Configuration and Training Objective}
For \textsc{ProcBERT}, we use the configuration \textsc{BERT}-base, which has 12 attention layers with 12 attention heads in each layer and the hidden dimension of 768. The training of \textsc{ProcBERT} involves two objectives, Masked Language Model (MLM) and Next Sentence Prediction (NSP). For \textsc{Proc-RoBERTa}, we continue pre-training \textsc{RoBERTa} on our collected procedural text following \citep{Gururangan2020DontSP}, so \textsc{Proc-RoBERTa} has the same configuration as \textsc{ProcBERT}, but its training only requires the MLM objective. 

\subsubsection{Tokenization \& Vocabulary}
% As the pre-training process requires document-level corpus, for those extracted paragraphs \FB{Need to be clearer.}, we treat each of them as one independent document. Besides, we segmented sentences with off-the-shelf NLP tools because sentence boundaries are important for the "next sentence prediction" task. Specifically, we used Scispacy \citep{Neumann2019ScispaCyFA} for PubMed articles and ChemDataExtractor \citep{Swain2016ChemDataExtractorAT} for chemical patents due to the domain relatedness.
As the sentence boundary is important for the NSP objective, we use the off-the-shelf NLP tools for sentence tokenization. Specifically, we used Scispacy \citep{Neumann2019ScispaCyFA} for PubMed articles and ChemDataExtractor \citep{Swain2016ChemDataExtractorAT} for chemical patents due to the domain relatedness.

In terms of the vocabulary, following BERT \citep{Devlin2019BERTPO} pre-processing procedure, we used the WordPiece tool provided from Huggingface Tokenizers\footnote{\url{https://github.com/huggingface/tokenizers}} \citep{Wolf2019HuggingFacesTS} to generate vocabulary for \textsc{ProcBERT} and thus tokenized our corpus. For \textsc{Proc-RoBERTa}, the original \textsc{RoBERTa} tokenizer is applied to our procedural text for pre-processing.  
% There are two important aspects in terms of vocabulary generation: 1) the corpus used to learn vocabulary; 2) the vocabulary size, which influences the split of Out-Of-Vocabulary tokens and the amount of parameters. As our focus is on procedural text understanding, we tried two setups, which are to generate the vocabulary using either the "original" procedural corpus or the "up-sampled" version. 
% As for the vocabulary size, we tried 30k and 50k, which are the vocabulary size of BERT \citep{Devlin2019BERTPO} and RoBERTa \citep{Liu2019RoBERTaAR} individually.

\subsubsection{Implementation}
\label{sec:implement}
We pre-train \textsc{ProcBERT} using the TensoFlow codebase of BERT\footnote{\url{https://github.com/google-research/bert}} \citep{Devlin2019BERTPO} from Google Research. We use Adam optimizer \citep{Kingma2015AdamAM} with $\beta_1$ = 0.9, $\beta_2$ = 0.999, $L2$ weight decay of 0.01. Following \citet{Devlin2019BERTPO}, we deploy the two-step regime to speed up our pre-traing. In the first step, we pre-train the model with sequence length 128 and batch size 512 for 1 million steps. The learning rate is warmed up over the first 100k steps to a peak value of 1e-4, then linearly decayed. In the second step, we train another 100k steps of sequence 512 and batch size 256 to learn the positional embeddings with peak learning rate 2e-5. We use the original subword mask as the mask strategy, and we mask 15\% of tokens in the sequence for both training steps.

For \textsc{Proc-RoBERTa}, we use the codebase of AI2\footnote{\url{https://github.com/allenai/tpu_pretrain}}, which enables pre-training the language model on TPU with PyTorch. Similar to \citep{Gururangan2020DontSP}, we train \textsc{RoBERTa} on our collected procedural text for 12.5k steps with the learning rate 3e-5 and the effective batch size 2048, which is archived by accumulating the gradient of 128 steps with the basic batch size 16. The input sequence length is 512 throughout the whole process, and 15\% words are masked for prediction as well.

\subsubsection{Model Variants}
To explore the effectiveness of these two models, we experiment with four variants. 
\paragraph{\textsc{Proc-RoBERTa-org}} We train \textsc{Proc-RoBERTa} on our \textbf{original} \textsc{Procedure} corpus as introduced above.
% in Section \ref{sec:implement}.
% For the first method of continuing fine-tuning the off-the-shelf language model, we present \textsc{Proc-RoBERTa}, which fine-tunes \textsc{RoBERTa} on our \textsc{Procedure} corpus as introduced in Section \ref{sec:implement}. 
\paragraph{\textsc{ProcBERT-org}} We train \textsc{ProcBERT} also on the \textsc{Procedure} corpus, and the vocabulary size is set to 50K for the fair comparison with \textsc{Proc-RoBERTa-org}.
% For the second method of pre-training a language model from scratch, we experiment with three variants, \textsc{ProcBERT-extract}, \textsc{ProcBERT-50K} and \textsc{ProcBERT-30K}. 

% \paragraph{\textsc{ProcBERT-50k} We train \textsc{ProcBERT} on the extended corpus \textsc{Procedure+} with two vocabulary sizes 50K and 30K to explore the best vocabulary size for our pre-trained language model.
\paragraph{\textsc{ProcBERT-50k}} We train \textsc{ProcBERT} on the extended corpus \textsc{Procedure+} with a vocabulary size of 50K.

\paragraph{\textsc{ProcBERT-30k}} This model uses the exactly same pre-training procedure as \textsc{ProcBERT-50k} with a smaller vocabulary size of 30K to see how the vocabulary size affects the pre-training.

Note that we did not experiment \textsc{Proc-RoBERTa} with the \textsc{Procedure+} corpus as 
% we thought \textsc{Proc-RoBERTa} might have some advantages when the size of the pre-training corpus is relatively small but 
\textsc{ProcBERT-org} already showed clear advantages over \textsc{Proc-RoBERTa-org} in Table \ref{tab:pretrain_results}.

\subsection{Fine-tuning Experiments}
\label{sec:downstream}
In this section, we present the performance of our pre-trained models on 5 procedural text-related downstream datasets, and compare them with off-the-shelf pre-trained language models.

\subsubsection{Downstream Tasks \& Datasets}
We experiment on Named Entity Recognition (NER), Relation Extraction (RE) and Entity Tracking (ET) three tasks to test the effectiveness of different in-domain pre-training strategies. NER is a sequence labeling task where the model detects named entity spans. RE is a classification task where the model predicts the relation between two entities in the same sentence. ET is a task of tracking the state change of entities over process steps. 

We experiment with 3 existing datasets \textsc{WLP}, \textsc{ChEMU}
% , \textsc{ProPara} 
and \textsc{Recipe}. Statistics, evaluation metrics and state-of-the-art models of all datasets can be found in Table~\ref{tab:task_statistics}. The \textsc{WLP} corpus provides entity and relation annotations for a collection of wet lab protocols. For named entity and relation extraction we follow the train/dev/test split from \citet{Tabassum2020WNUT2020T1}. The \textsc{ChEMU} corpus \citep{Nguyen2020ChEMUNE} provides entity and event annotations for 1500 chemical reaction snippets collected from 170 English patents. 
% The \textsc{ProPara} dataset \citep{Dalvi2018TrackingSC} includes the state changes and locations of entities in the scientific process for 488 human-written paragraphs. 
The \textsc{Recipe} \citep{Kiddon2016GloballyCT} dataset includes the annotation of involved ingredients of each cooking step for 866 recipes.

% \FB{Add a section that motivates two new datasets (details in Appendix)} 
As mentioned in Section \ref{sec:intro}, one major contribution of this paper is to compare pre-training based approaches with supervised domain adaptation approaches. Therefore, to accommodate the supervised domain adaptation setting, we created two new datasets \textsc{PubMedM\&M} and \textsc{ChemSyn} in the domain of scientific articles and chemical patents mainly following the annotation scheme of the Wet Lab Protocols (WLP) framework \citep{Kulkarni2018AnAC} with 4 entity types and 1 relation type added  (more details of data annotation are shown in Appendix \ref{sec:data_anno}). 
% In WLP, there are 18 Entity types (including the Action) and 14 Relation types. On top of it, we supplemented four new Entity types (\textsc{Company}, \textsc{Software}, \textsc{Collection(Data)} and \textsc{Info-Type}) and one new Relation type (\textsc{Belong-To}) due to two key features of our corpus: 1) Scientific articles usually specify the provenance of reagents for better reproducibility; 2) Other than wet-lab experiments, our corpus also includes the detail of data processing/analysis and computer-simulated experiments. 
For the \textsc{PubMedM\&M} dataset, we annotated a corpus of 191 procedural text paragraphs sampled from all extracted PubMed procedural paragraphs (Appendix \ref{sec:app_corpus}). Similarly, for the \textsc{ChemSyn} dataset, we annotated 600 chemical synthesis-related paragraphs, and used 596 paragraphs for experiments after removing 4 duplicate ones. 
% The annotation detail and the inter-annotator agreement score can be found in  \FB{This should be moved earlier.}.
% The annotation process is conducted with BRAT annotation tool, and it consists of two steps. In the first step, each file is distributed to two annotators, and they will annotate the file independently. Then in the second step, the coordinator will discuss the annotation with each annotator making sure their annotation follows the guideline and dissolve the disagreement. We double-annotated all files in the \textsc{PubMedM\&M} dataset and half of the files in the \textsc{ChemSyn} dataset. As for the inter-annotator agreement (IAA) score, we treat the annotation from one of the two annotator as the gold label, and the other annotation as the predicted label, and then use the F1 scores of Entity(Action) and Relation evaluations as the final inter-annotator agreement scores, which can be found in Table \ref{tab:iaa_results}. We can see that the \textsc{ChemSyn} dataset has higher IAA scores for two potential reasons: 1) we annotated the \textsc{PubMedM\&M} dataset first, so the annotators might be more experienced when they annotated the \textsc{ChemSyn} dataset; 2) the \textsc{PubMedM\&M} dataset contains more diverse content like wet lab experiments or computer simulation procedures while the \textsc{ChemSyn} dataset is mainly about chemical synthesis.

\begin{table*}[t!]
\small
\begin{center}
% \setlength\tabcolsep{1pt}
\resizebox{\textwidth}{!}{\begin{tabular}{ccccccccc}
\thickhline Dataset & Domain & Task & \#Files & \#Sentences & \#Cases & \#Classes & Metric & SOTA Model\\ \hline
\multirow{2}{*}{\textsc{WLP}   \citep{Tabassum2020WNUT2020T1}}         & \multirow{2}{*}{biology}
  & NER    & \multirow{2}{*}{615} & \multirow{2}{*}{14,096} & 80,659 & 19 & $F_1$ & \citet{Knafou2020BiTeMAW} \\
& & RE     &                      &                         & 54,212 & 16 & $F_1$ & \citet{Sohrab2020mgsohrabAW} \\ \hline
\multirow{2}{*}{\textsc{X-WLP} \citep{tamari-etal-2021-process-level}} & \multirow{2}{*}{biology}
  & MI+PG   & -                    & -                       & -      & 11 & $F_1$ \\
& & ARL+TO & -                    & -                       & -      & -  & $F_1$ \\ \hline
% \textsc{ProPara} \citep{Dalvi2018TrackingSC} & science & ET & 488 & 3,273 & 13,117 & 4 & Cat-2 \\ \hline
\textsc{Recipe} \citep{Kiddon2016GloballyCT}                           & life 
  & ET     & 866                  & 7,648                   & 74,004 & 2  & Acc.  & \citet{Gupta2019EffectiveUO}\\ \hline
\multirow{2}{*}{\textsc{ChEMU} \citep{Nguyen2020ChEMUNE}}              & \multirow{2}{*}{chem.}
  & NER    & -                    & -                       & -      & 11 & $F_1$ \\
& & EE     & -                    & -                       & -      & -  & $F_1$ \\ \hline
% \multirow{4}{*}{Proposed} &
\multirow{2}{*}{\textsc{PubMedM\&M} (this work)}         & \multirow{2}{*}{biomed.}
  & NER    & \multirow{2}{*}{191} & \multirow{2}{*}{1,508}  & 12,131 & 23 & $F_1$ & - \\
& & RE     &                      &                         & 8,987  & 17 & $F_1$ & - \\ \hline
\multirow{2}{*}{\textsc{ChemSyn} (this work)}                          & \multirow{2}{*}{chem.}
  & NER    & -                    & -                       & -      & 23 & $F_1$ & - \\
& & RE     & -                    & -                       & -      & 17 & $F_1$ & - \\ \thickhline
\end{tabular}}
\end{center}
\caption{\label{tab:task_statistics}Statistics of 5 downstream datasets.}
\end{table*}

\subsubsection{Experimental Setup}
We follow the experimental setup of the respective paper for each task, and report averages and standard deviations across five random seeds for all our experiments. 
For NER in four related datasets, a prediction is correct only if its label and boundary both match with the gold entity mention, and we use the Perl script \texttt{conlleval}\footnote{\url{https://www.clips.uantwerpen.be/conll2000/chunking/output.html}} for evaluation. For RE in three corresponding datasets, as we only consider the case where the input is gold entity mentions, a relation prediction is correct when its label matches with the gold relation. 
% For EE, we follow the setup of \citet{Nguyen2020ChEMUNE}, where we only need to identify the event trigger and 
We use $F_1$ score as the evaluation metric for both NER and RE. 
Note that in the \citet{Tabassum2020WNUT2020T1} version of the \textsc{WLP}, the dataset is split into four subsets randomly: train, dev, test, and test-2020 (used as the final test data for the shared task) , so we follow the setup of the top-performing system \textsc{mgsohrab} \citep{Sohrab2020mgsohrabAW} in the shared task, to merge the original train and dev as the new train set, and treat test and test-2020 as the new dev and test set respectively. 

For ET, we follow the setup of \citet{Gupta2019EffectiveUO}, where the model predicts the state of the entity at each timestep of the procedure from a set of pre-defined classes. These classes are 
% create (C), move(M), destroy (D) and none (O) for the \textsc{ProPara} dataset, and 
the presence (1) or absence (0) for the \textsc{Recipe} dataset.  
% For the \textsc{ProPara} dataset, we use the standard evaluation scheme, which is framed as answering the following categories of questions: (Cat-1) Is e created (destroyed, moved) in the process; (Cat-2) When (step #) is e created (destroyed, moved)? 
For the \textsc{Recipe} dataset, the evaluation metric is the accuracy. 

\subsubsection{Baselines}
As for the baselines, we use the off-the-shelf domain-agnostic LMs \textsc{BERT}-base-uncased \citep{Devlin2019BERTPO} and \textsc{RoBERTa}-base \citep{Liu2019RoBERTaAR} for all datasets. We also experiment with \textsc{SciBERT} \citep{Beltagy2019SciBERTAP} and \textsc{BioMed-RoBERTa} \citep{Gururangan2020DontSP} to see how our proposed models compare with other strong domain-specific pre-trained language models. 

% To show the effectiveness of different domain-specific pre-training strategies, we present four models. 
% \paragraph{\textsc{Proc-RoBERTa-org}} We train \textsc{Proc-RoBERTa} on our \textbf{original} \textsc{Procedure} corpus as introduced in Section \ref{sec:implement}.
% For the first method of continuing fine-tuning the off-the-shelf language model, we present \textsc{Proc-RoBERTa}, which fine-tunes \textsc{RoBERTa} on our \textsc{Procedure} corpus as introduced in Section \ref{sec:implement}. 
% \paragraph{\textsc{ProcBERT-org}} We train \textsc{ProcBERT} on the \textsc{Procedure} corpus, and the vocabulary size is set to 50K for the fair comparison with \textsc{Proc-RoBERTa-org}.
% For the second method of pre-training a language model from scratch, we experiment with three variants, \textsc{ProcBERT-extract}, \textsc{ProcBERT-50K} and \textsc{ProcBERT-30K}. 
% \paragraph{\textsc{ProcBERT-50k} and \textsc{ProcBERT-30k}} We train \textsc{ProcBERT} on the extended corpus \textsc{Procedure+} with two vocabulary sizes 50K and 30K to explore the best vocabulary size for our pre-trained language model.

% Note that we did not experiment \textsc{Proc-RoBERTa} with the \textsc{Procedure+} corpus as 
% we thought \textsc{Proc-RoBERTa} might have some advantages when the size of the pre-training corpus is relatively small but 
% \textsc{ProcBERT-org} already showed clear advantages over \textsc{Proc-RoBERTa-org} in Table \ref{tab:pretrain_results}.

% We present four procedural text pre-trained language models. 
% \textsc{ProcBERT}-extract and \textsc{Proc-RoBERTa} are two models trained on the original corpus \textsc{Procedure}, which mostly consists of extracted procedural paragraphs from full documents.
% On the smaller corpus \textsc{Procedure}, we experiment with both in-domain pre-training strategies introduced previously. As the \textsc{Procedure} corpus mostly consists of extracted paragraphs, we named the pre-trained model \textsc{ProcBERT}-extract for the pre-training from scratch and \textsc{Proc-RoBERTa} for continuing fine-tuning the \textsc{RoBERTa}
% For our proposed procedural text pre-training, we experimented with three setups: 1) Similar to \citet{Gururangan2020DontSP}, we fine-tuned the RoBERTa-base model on our extracted procedural corpus for 100k step with the batch size 128 (denoted as Proc-RoBERTa); 2) We pre-trained the LM from scratch only using extracted corpus (denoted as ProcBERT-extract); 3) We pre-trained the LM from scratch using the "up-sampled" version of procedural corpus with two vocabulary sizes (denoted as ProcBERT-30k and ProcBERT-50k). 
% \FB{Miss the introduction to SOTA models on the selected datasets.}

\subsubsection{Fine-tuning Architecture}
\label{sec:finetune_arc}
We use a different fine-tuning architecture for each task. For NER, we follow \citet{Devlin2019BERTPO} to feed the final contextualized embedding of each token into
a linear classification layer with softmax output. For RE, our architecture is similar to \citet{Soares2019MatchingTB}, where four special tokens \texttt{[E1]}, \texttt{[\textbackslash E1]}, \texttt{[E2]}, \texttt{[\textbackslash E2]} are used to specify the positions of two entities, and the contextualized embeddings of \texttt{[E1]} and \texttt{[E2]} are concatenated as input to a final linear layer that is used to predict the relation. For ET, following \citet{Gupta2019EffectiveUO}, our model uses the query entity and the whole procedure paragraph as the input. We concatenate query entity and all sentences in the paragraph together while adding two special tokens \texttt{[CLS]} and \texttt{[SEP]} at the start and end of each sentence. We then use the contextualized embedding of \texttt{[CLS]} to predict the state change of the query entity for each procedural step.

All models are implemented using Huggingface Transformers \citep{Wolf2019HuggingFacesTS}. We use AdamW as the optimizer for all the experiment, and pick the best learning rate, batch size and number of epochs on the development set and report the corresponding test results (see Appendix \ref{sec:hyper_para} for more details about hyper-parameters). 

\subsubsection{Results}
The results of all models on 5 datasets are presented in Table \ref{tab:pretrain_results}. 
As we can see, both \textsc{Proc-RoBERTa-org} and \textsc{ProcBERT-org} 
% \FB{Model names should be fixed.} 
can outperform their domain-agnostic counterparts \textsc{RoBERTa} and \textsc{BERT} in all datasets showing the effectiveness of in-domain pre-training.
The strategy of pre-training a language model from scratch seems to lead to a better domain-specific language model compared to fine-tuning the off-the-shelf pre-trained language models as \textsc{ProcBERT-org} works better than \textsc{Proc-RoBERTa-org}, and \textsc{SciBERT} works better than \textsc{BioMed-RoBERTa} in most cases. 
There are two possible reasons: 1) Pre-training from scratch uses a customized vocabulary, which captures important domain-specific information; 2) Following \citet{Gururangan2020DontSP}, \textsc{RoBERTa} is only in-domain fine-tuned for 12.5k steps with the batch size of 2048, computationally equal to fine-tuning \textsc{RoBERTa} for 100k steps with the batch size of 256, which is far less than the computation of pre-training a language model from scratch suggesting that the prevailing fine-tuning strategy from \citep{Gururangan2020DontSP} may still leave the language model under-trained. 
After using the bigger corpus \textsc{Procedure+} for pre-training, the performance of \textsc{ProcBERT} get improved. 
It outperforms many baselines like \textsc{SciBERT} and \textsc{BioMed-RoBERTa} (marginally for some tasks), and even archives the state-of-the-art performance on multiple tasks like RE for the WLP dataset and ET for the Recipe dataset.
% In terms of the vocabulary size, the bigger vocabulary does not always lead to a better performance mainly because our pre-training corpus is not big enough compared to the pre-training corpus of \textsc{RoBERTa}. 
% Moreover, all our procedural text-pre-trained models do not succeed on the \textsc{ProPara} dataset as the paragraphs in this dataset are written by the crowdsourcing annotators, which may have totally different language distribution compared to our collected corpus.
Interestingly, we notice that, for the \textsc{Recipe} dataset, \textsc{ProcBERT-30k} and \textsc{ProcBERT-50k} perform worse than \textsc{ProcBERT-org}, and we think it is mainly because the proportion of recipe text is diluted in \textsc{Procedure+}.



\begin{table*}[t!]
\small
\begin{center}
% \setlength\tabcolsep{1pt}
\resizebox{\textwidth}{!}{\begin{tabular}{cccccccccccc}
\thickhline 
% Name & \multicolumn{2}{c}{\bf\textsc{WLP}} & \multicolumn{2}{c}{\bf\textsc{PubMedM\&M}} & \multicolumn{1}{c}{\bf\textsc{ChEMU}} & \multicolumn{2}{c}{\bf\textsc{ChemSyn}} & \bf\textsc{ProPara} & \bf\textsc{Recipe}  \\ 
% & \multicolumn{1}{c}{\textsc{NER}} & \multicolumn{1}{c}{\textsc{RE}} & \multicolumn{1}{c}{\textsc{NER}} & \multicolumn{1}{c}{\textsc{RE}} & \multicolumn{1}{c}{\textsc{NER}}  &  \multicolumn{1}{c}{\textsc{NER}} & \multicolumn{1}{c}{\textsc{RE}} & ET & ET \\ \hline
% \textsc{BERT} \citep{Devlin2019BERTPO}               & 74.33$\pm$0.1    & 80.25$\pm$0.4    & 70.71$\pm$0.3    & 78.73$\pm$0.9    &                  & 93.64$\pm$0.3    & 91.95$\pm$0.3    & 53.37$\pm$0.7    & 80.62$\pm$0.7 \\ 
% \textsc{RoBERTa} \citep{Liu2019RoBERTaAR}            & 75.29$\pm$0.3    & 80.94$\pm$0.5    & 72.20$\pm$0.5    & 78.95$\pm$0.7    &                  & 94.00$\pm$0.3    & 92.62$\pm$0.3    & \bf55.49$\pm$1.0 & 83.41$\pm$0.1 \\ 
% \textsc{SciBERT} \citep{Beltagy2019SciBERTAP}        & 76.36$\pm$0.3    & 81.29$\pm$0.5    & 73.61$\pm$0.3    & 79.54$\pm$0.9    & \bf00.00$\pm$0.0 & 94.55$\pm$0.1    & 92.40$\pm$0.3    & 53.90$\pm$0.6    & - \\ 
% \textsc{BioMed-RoBERTa} \citep{Gururangan2020DontSP} & 75.50$\pm$0.3    & 81.56$\pm$ 0.4   & 73.26$\pm$0.4    & 78.44$\pm$2.0    &                  & 94.13$\pm$0.2    & 92.54$\pm$0.3    & -                & - \\ \hline
% \textsc{Proc-RoBERTa-org}                            & 75.57$\pm$0.5    & 80.79$\pm$0.9    & 72.91$\pm$0.6    & 78.51$\pm$1.0    &                  & 94.66$\pm$0.3    & 92.81$\pm$0.4    & TODO             & 84.19$\pm$0.3\\
% \textsc{ProcBERT-org}                                & 76.34$\pm$0.4    & 81.65$\pm$0.5    & 73.64$\pm$0.4    & 79.46$\pm$0.4    &                  & \bf95.20$\pm$0.2 & 92.99$\pm$0.2    & TODO             & \bf84.54$\pm$0.3 \\
% \textsc{ProcBERT-50k}                                & 76.43$\pm$0.2    & \bf81.94$\pm$0.4 & 73.64$\pm$0.5    & \bf80.26$\pm$0.7 &                  & 95.07$\pm$0.2    & 92.85$\pm$0.1    & 54.83$\pm$2.6    & 83.90$\pm$0.3 \\
% \textsc{ProcBERT-30k}                                & \bf76.56$\pm$0.5 & 81.44$\pm$0.4    & \bf73.75$\pm$0.5 & 80.19$\pm$0.6    &                  & 95.07$\pm$0.1    & \bf93.13$\pm$0.3 & TODO             & 84.10$\pm$0.3 \\
%  \hline
% \textsc{SOTA}                      & 77.99            & 80.46            & -               & -                &                  & -                 & - \\ \thickhline
                          & \multicolumn{2}{c}{\bf\textsc{WLP}} & \multicolumn{2}{c}{\bf\textsc{X-WLP}} & \multicolumn{2}{c}{\bf\textsc{PubMedM\&M}} & \multicolumn{2}{c}{\bf\textsc{ChEMU}} & \multicolumn{2}{c}{\bf\textsc{ChemSyn}} & \bf\textsc{Recipe}  \\ 
Model Name                & \multicolumn{1}{c}{\textsc{NER}} & \multicolumn{1}{c}{\textsc{RE}} & \multicolumn{1}{c}{\textsc{NER}} & \multicolumn{1}{c}{\textsc{RE}} & \multicolumn{1}{c}{\textsc{NER}} & \multicolumn{1}{c}{\textsc{RE}} & \multicolumn{1}{c}{\textsc{NER}}  &  \multicolumn{1}{c}{\textsc{RE}} & \multicolumn{1}{c}{\textsc{NER}} & \multicolumn{1}{c}{\textsc{RE}} & ET \\ \hline
\textsc{BERT}             & 
74.33$\pm$0.1    & 80.25$\pm$0.4    &                  &                  & 70.71$\pm$0.3    & 
78.73$\pm$0.9    &                  &                  & 93.64$\pm$0.3    & 91.95$\pm$0.3    & 80.62$\pm$0.7   \\ 
\textsc{RoBERTa}          & 
75.29$\pm$0.3    & 80.94$\pm$0.5    &                  &                  & 72.20$\pm$0.5    & 
78.95$\pm$0.7    &                  &                  & 94.00$\pm$0.3    & 92.62$\pm$0.3    & 83.41$\pm$0.1   \\ 
\textsc{SciBERT}          & 
76.36$\pm$0.3    & 81.29$\pm$0.5    & \bf00.00$\pm$0.0 & \bf00.00$\pm$0.0 & 73.61$\pm$0.3    & 
79.54$\pm$0.9    & \bf00.00$\pm$0.0 & \bf00.00$\pm$0.0 & 94.55$\pm$0.1    & 92.40$\pm$0.3    & -               \\ 
\textsc{BioMed-RoBERTa}   & 
75.50$\pm$0.3    & 81.56$\pm$ 0.4   &                  &                  & 73.26$\pm$0.4    & 
78.44$\pm$2.0    &                  &                  & 94.13$\pm$0.2    & 92.54$\pm$0.3    & -                \\ \hline
\textsc{Proc-RoBERTa-org} & 
75.57$\pm$0.5    & 80.79$\pm$0.9    &                  &                  & 72.91$\pm$0.6    & 
79.16$\pm$0.9    &                  &                  & 94.66$\pm$0.3    & 92.81$\pm$0.4    & 84.19$\pm$0.3    \\
\textsc{ProcBERT-org}     & 
76.34$\pm$0.4    & 81.65$\pm$0.5    &                  &                  & 73.64$\pm$0.4    & 
79.46$\pm$0.4    &                  &                  & \bf95.20$\pm$0.2 & 92.99$\pm$0.2    & \bf84.54$\pm$0.3 \\
\textsc{ProcBERT-50k}     & 
76.43$\pm$0.2    & \bf81.94$\pm$0.4 &                  &                  & 73.64$\pm$0.5    & 
\bf80.26$\pm$0.7 &                  &                  & 95.07$\pm$0.2    & 92.85$\pm$0.1    & 83.90$\pm$0.3    \\
\textsc{ProcBERT-30k}     & 
\bf76.56$\pm$0.5 & 81.44$\pm$0.4    &                  &                  & \bf73.75$\pm$0.5 & 
80.19$\pm$0.6    &                  &                  & 95.07$\pm$0.1    & \bf93.13$\pm$0.3 & 84.10$\pm$0.3    \\
 \hline
\textsc{SOTA}             & 
77.99            & 80.46            &                  &                  & -               & 
-                &                  & -                 & - \\ \thickhline
\end{tabular}}
\end{center}
\caption{\label{tab:pretrain_results}Results.}
\end{table*}

==> sections_old/3_label.tex <==
\begin{figure}
\includegraphics[width=8cm]{figures/chemsyn_ner_budget.pdf}
\caption{\label{fig:budget} Results.}
\end{figure}

% In the previous section, we show that an in-domain pre-trained language model can greatly improve the downstream task performance especially when it is pre-trained from scratch with a customized vocabulary. 
% In the previous section, we show that an in-domain pre-trained language model can greatly improve the downstream task performance especially when it is pre-trained from scratch with a customized vocabulary.
In the previous section, we investigate pre-training-based domain adaptation on procedural text understanding.
% as the first step to research the applicability of domain adaptation methods.
% However, one non-negligible down side of this model is its training requires a large amount of computation, which leads to prohibitive cost \citep{Strubell2019EnergyAP}.
% In this section, we explore how we can efficiently take advantage of the annotated data while using the pre-trained language model to boost the target task. \FB{This section needs to be improved.}
% In this section, we explore supervised domain adaptation, an effective alternative of the pre-training-based unsupervised approach, where we study how to efficiently use the labeled data to boost the target domain task.
% In this section, we compare unsupervised domain adaptation with supervised domain adaptation.
In this section, we compare it with supervised domain adaptation methods, which uses labeled data to boost a target domain task, considering both cost and performance.
% As an effective alternative of the unsupervised domain adaptation, the supervised domain adaptation uses labeled data to boost a target domain task.
% Specifically, we first explore the classic supervised domain adaptation framework \textsc{EasyAdapt} and then put it into a budget-aware comparison with the best-performing unsupervised method in Section \ref{sec:pre-train}.
% In this way, we can understand the applicability of these two types of domain adaptation methods better in practice.
Specifically, we first introduce \textsc{EasyAdapt}, a classic supervised domain adaptation framework, and then include it and the simple task-specific annotation method \textsc{Annotate} together with the two methods mentioned above into a budget-aware comparison to see which one works the best in practice.


% In this section, we explore how to use the labeled data, as an effective alternative of the unsupervised pre-training-based approach, to boost the target domain task.
% where we study how to efficiently use the annotated data with the domain-agnostic pre-trained language model to boost the target domain task.


% \subsection{DA with Out-of-domain Labeled Data}
% \subsection{Out-of-domain Labeled Data}
% \subsection{Supervised Domain Adaptation}
\subsection{EasyAdapt}
% compare the prevailing in-domain pre-training technique with the simple data annotation method, and 
% As we show in the previous sub-section, collecting in-domain labelled data is more important than pre-training given a lower budget. In this sub-section, we explore the traditional supervised domain adaptation method and compare it with the in-domain pre-training as it can utilize out-of-domain labeled data effectively without further cost.
% and how we can use both methods to further boost the performance.

% \subsubsection{Problem Formulation and Background}
For supervised domain adaptation, we have access to labeled corpus for source domain $D^s$ and target domain $D^t$, and we want to use both datasets to achieve the best performance on the target data.
Although many successful supervised domain adaptation methods have been proposed, in this paper, we focus on the simple but effective feature augmentation framework \textsc{EasyAdapt} \citep{Daum2007FrustratinglyED}, which sets up a distinct feature space for each domain and creates a separate feature space shared across all domains so that the knowledge can be transferred via this shared feature space.
Previous works \citep{Kim2016FrustratinglyEN, Peng2017MultitaskDA} extended it by using neural networks like LSTM as the feature generator. Here we show how to incorporate the prevalent pre-trained language model in the context of procedural text understanding.

\subsubsection{Model}
% We now describe our proposed method,
% \textbf{P}re-trained \textbf{L}anugage \textbf{M}odel-based \textbf{F}eature \textbf{A}ugmentation (\textsc{PLMFA}), 
% which uses a pre-trained language model as the representation learner for the \textsc{EasyAdapt} framework, and can be applied to both NER and RE two tasks.
We now describe how our proposed method is applied
% , which is an extension of the \textsc{EasyAdapt} framework using a pre-trained language model, and can be applied to
to NER and RE two tasks.
We first generate the feature representation of the input sequence.
For NER, it is the hidden vector generated from the last layer of the pre-trained language model for each word. For RE, it is the concatenation of contextual embeddings of special tokens \texttt{[E1]} and \texttt{[E2]} as introduced in \S\ref{sec:finetune_arc}.
Once we have the feature vector, the next step in \textsc{EasyAdapt} is to build an augmented feature space.
% Suppose we have one source domain, one target domain and one shared domain, we build the augmented feature space by replicating the feature vector three times and use one feature vector to represent a distinct domain. 
Suppose we have one source domain and one target domain, we replicate the feature vector three times as the augmented feature representation, where first two vectors represent the source and target domain respectively, and the last vector represents a shared feature space, which is used for knowledge transfer.
Given a data point from one specific domain (source or target), we concatenate the feature vector of its own domain and the feature vector of the shared domain as the input to a linear classification layer for both NER and RE two tasks. 


% \paragraph{NER} We use the hidden vector generated from the final layer of the pre-trained language model for each word's representation, which is denoted as:
% % \small
% \begin{equation}
% h_t = \texttt{PLM}(x_{1:n}, t)
% \label{eq:h_word}
% \end{equation}
% \normalsize

% \noindent where $x_{1:n}$ means the input sentence of the length $n$, $t$ denotes the word position, and PLM could be a domain-agnostic pre-trained language model like \textsc{BERT}, or a domain-specific one like \textsc{ProcBERT-30k}. Therefore, the representation for the input sentence is denoted as: 
% % \small
% \begin{equation}
% \mathbf{h} = h_{1:n}
% \label{eq:h_ner}
% \end{equation}
% \normalsize

% \paragraph{RE} Introduced in Section \ref{sec:finetune_arc}, we use the concatenation of contextual embeddings of special tokens \texttt{[E1]} and \texttt{[E2]} as the final representation of the input sequence denoted as:
% % \small
% \begin{equation}
% \mathbf{h} = [\texttt{PLM}(x_{1:n}, t_{[E1]});\texttt{PLM}(x_{1:n}, t_{[E2])}]
% \label{eq:h_re}
% \end{equation}
% \normalsize

% \noindent where $t_{[E1]}$ and $t_{[E2]}$ denotes the positions of special tokens \texttt{[E1]} and \texttt{[E2]}. 

% Once we have the feature vector, the next step is to build the augmented feature space. We implement this idea via the domain masking strategy similar to \citet{Peng2017MultitaskDA}. 
% % owever, the difference is, instead of segmenting the feature representation into multiple sections, we extend the original feature space with two methods depending on how we choose the PLM. 
% Suppose we have one source domain and one target domain, 
% % and we want to create three feature spaces for the source, the target and the shared domain. 
% % If we only use one pre-trained language model for all domains, the augmented feature vector would be:
% the augmented feature vector including all three domain is denoted as:
% % \small
% % \begin{equation}
% % % \mathbf{h}_{aug} = [\mathbf{h}_{\textrm{PLM}};\mathbf{h}_{\textrm{PLM}};\mathbf{h}_{\textrm{PLM}}]
% % \mathbf{h}_{aug} = [\mathbf{h};\mathbf{h};\mathbf{h}]
% % \label{eq:h_mlm_one}
% % \end{equation}
% % \normalsize

% % \noindent However, if we have one specific pre-trained language model for each feature space, the augmented feature vector would be:
% % % \small
% \begin{equation}
% \mathbf{h}_{aug} = [\mathbf{h}_{src};\mathbf{h}_{tgt};\mathbf{h}_{sha}]
% \label{eq:h_mlm_multi}
% \end{equation}
% \normalsize
% \noindent where $\mathbf{h}$ denotes the feature vector generated in Equation \ref{eq:h_ner} or Equation \ref{eq:h_re} for each feature space. The mask for source and target domains would be:
% % \small
% \begin{equation}
% \mathbf{m}_{src} = [\vec{1}, \vec{0}, \vec{\alpha}], \quad \mathbf{m}_{tgt} = [\vec{0}, \vec{1}, \vec{1}]
% % \mathbf{m}_{src} = [\vec{1}, \vec{0}, \vec{1}], \quad \mathbf{m}_{tgt} = [\vec{0}, \vec{1}, \vec{1}]
% \label{eq:mask}
% \end{equation}
% \normalsize
% \noindent where $\alpha$ is a tunable hyper-parameter, which makes the feature vector of the shared space domain-agnostic.
% % control the effect of two datasets on the shared feature space as the amounts of annotated data from two datasets are imbalanced.  
% We can then use the mask vector to generate the final feature vector $\hat{\mathbf{h}}$:

% % \small
% \begin{equation}
% \hat{\mathbf{h}} = \mathbf{h}_{aug} \odot \mathbf{m}
% \label{eq:h_hat}
% \end{equation}
% \normalsize

% \noindent where $\odot$ denotes element-wise multiplication. Those augmented feature vectors $\hat{\mathbf{h}}$ replace the original $\mathbf{h}$ as the input to a linear classification layer for both NER and RE two tasks. Note that the dimension of the linear layer now becomes three times as large.

\subsubsection{Experimental Setup}
% We use \textsc{WLP}, \textsc{PubMedM\&M} and \textsc{ChemSyn} for our supervised domain adaptation experiments and treat \textsc{WLP} and \textsc{ChemSyn} as the source domain respectively and \textsc{PubMedM\&M} as the target domain because \textsc{WLP} and \textsc{ChemSyn} have much more annotated data compared to \textsc{PubMedM\&M}. 
We use \textsc{WLP}, \textsc{PubMedM\&M} and \textsc{ChemSyn} all three datasets for our supervised domain adaptation experiments.
As \textsc{PubMedM\&M} has relatively less data, we did not use it as the source domain.
Besides, \textsc{PubMedM\&M} and \textsc{ChemSyn} includes new entity and relation types, which do not exist in \textsc{WLP}, so we use shared entity and relation types in our experiments. 
% Note that as mentioned by \citet{Daum2007FrustratinglyED} the amount of target labeled data should be "enough to do slightly better than just using 'source' data", and Table \ref{tab:da_results} shows that this assumption ("slightly") does not hold, we still uses all target domain data to see if the proposed model can work in such a extreme setup.
The data statistics of three datasets can be found in Table \ref{tab:sda_stats}. 
% As for the pre-trained language model, we experiment with two models, one domain-general BERT and one domain-sensitive ProcBERT-50K.

\begin{table}[h!]
\small
\begin{center}
% \setlength\tabcolsep{3pt}
\begin{tabular}{ccccccc}
\thickhline  & \multicolumn{2}{c}{\textsc{WLP}} & \multicolumn{2}{c}{\textsc{ChemSyn}} & \multicolumn{2}{c}{\textsc{PubMedM\&M}} \\ 
& NER & RE & NER & RE & NER & RE \\ \hline
train &  &  &  &  &  &\\ 
dev & & & & &  & \\ 
test & & & & &  & \\ 
\thickhline
\end{tabular}
\end{center}
\caption{\label{tab:sda_stats}  Statistics of the \textsc{WLP}, \textsc{ChemSyn} and \textsc{PubMedM\&M} in supervised domain adaptation experiments.}
\end{table}

% \subsubsection{Baselines}
In terms of baselines, we include three simple but "tough-to-beat" methods:
% We include three simple but "tough-to-beat" baselines and present two model variations: 
% (especially when the size of labeled target data is relatively large):
\paragraph{\textsc{OnlySRC}} We only use the labeled data from the source domain for model training.
\paragraph{\textsc{OnlyTGT}} We ignore the source domain data and only use target domain data for training.
\paragraph{\textsc{Combine}} We combine the training sets of both source and target domains to train a model.
% \paragraph{\textsc{PLMFA-One}} We use one pre-trained language model to generate features for all domains in \textsc{PLMFA}.
% \paragraph{\textsc{PLMFA-Multi}} We use a separate pre-trained language model for each domain in \textsc{PLMFA}.

\subsubsection{Results}
The test set results of all four methods are presented in Table \ref{tab:sda_results}. 
We can see that \textsc{OnlyTGT} always outperforms \textsc{OnlySRC} despite the smaller size of training data in the target domain demonstrating the importance of in-domain labeled training data. 
\textsc{Combine} works better than \textsc{OnlyTGT} in most cases but worse on the NER task when \textsc{WLP} is the source dataset showing that mixing the training data from two different domains might hurt the performance on the target domain. 
% \FB{Maybe I should add more explanation on why performance gets worse here.} 
Our proposed model, which integrates the pre-trained language model into the \textsc{EasyAdapt} framework, outperforms all the baselines.
\textsc{EasyAdapt} achieves the best overall results when working with \textsc{ProcBERT} illustrating that the pre-training-based domain adaptation and supervised domain adaptation can work well together to further elevate the performance of the downstream tasks. 
% This illustrates that: 1) The domain-specific pre-training and supervised domain adaptation can work well together to elevate the performance of the downstream tasks; 2) Having a separate pre-trained language model to generate features for each domain is important to utilizing labeled data effectively from multiple domains. 
Interestingly, in some scenarios, such as the RE task when \textsc{WLP} is the source dataset, the performance gain from our proposed \textsc{EasyAdapt} can surpass the performance gains from the in-domain pre-training, which signals the potential of supervised domain adaptation approaches. 
% Moreover, the domain-specific language model and supervised domain adaptation method can work well together to further elevate the performance of the downstream tasks to a new level.

\begin{comment}
\begin{table*}[t!]
\small
\begin{center}
% \setlength\tabcolsep{1pt}
\resizebox{\textwidth}{!}{\begin{tabular}{ccccccccccc}
\thickhline 
% & \multirow{2}{*}{Models} & \multicolumn{6}{c}{Datasets} \\
& \multicolumn{4}{c}{\bf\textsc{WLP}} & \multicolumn{4}{c}{\bf\textsc{ChemSyn}} \\
 & \multicolumn{2}{c}{NER} & \multicolumn{2}{c}{RE} & \multicolumn{2}{c}{NER} & \multicolumn{2}{c}{RE}  \\ 
& \multicolumn{1}{c}{\textsc{BERT}} & \multicolumn{1}{c}{\textsc{ProcBERT}} & \multicolumn{1}{c}{\textsc{BERT}} & \multicolumn{1}{c}{\textsc{ProcBERT}} & \multicolumn{1}{c}{\textsc{BERT}} & \multicolumn{1}{c}{\textsc{ProcBERT}} & \multicolumn{1}{c}{\textsc{BERT}} & \multicolumn{1}{c}{\textsc{ProcBERT}} \\ \hline
\textsc{EasyAdapt} & \bf72.61$\pm$0.7 & \bf74.77$\pm$0.4 & \bf79.99$\pm$0.6 & \bf81.22$\pm$0.3 & \bf72.91$\pm$0.4 & \bf75.16$\pm$0.2 & \bf78.91$\pm$0.5 & \bf80.47$\pm$0.6 \\ \hline
\textsc{OnlySRC} & 60.91$\pm$1.0 & 63.65$\pm$0.5 & 73.09$\pm$0.6 & 74.28$\pm$0.7 & 65.27$\pm$0.7 & 68.04$\pm$0.5 & 71.38$\pm$0.5 & 73.61$\pm$0.7 \\ 
\textsc{OnlyTGT} & 72.45$\pm$0.3 & 74.55$\pm$0.2 & 77.54$\pm$0.8 & 79.95$\pm$0.4 & 72.45$\pm$0.3 & 74.55$\pm$0.2 & 77.54$\pm$0.8 & 79.95$\pm$0.4 \\ 
\textsc{Combine} & 70.73$\pm$0.2 & 73.96$\pm$0.4 & 79.02$\pm$0.3 & 79.84$\pm$0.7 & 72.91$\pm$0.5 & 75.14$\pm$0.3 & 78.28$\pm$0.6 & 80.30$\pm$0.7 \\ 
% \textsc{PLMFA-Multi} & \bf73.20$\pm$0.5 & \bf74.97$\pm$0.3 & & & \bf73.37$\pm$0.4 & \bf75.42$\pm$0.4 \\ 
\thickhline
\end{tabular}}
\end{center}
\caption{\label{tab:sda_results}Results. }
\end{table*}
\end{comment}

\begin{comment}
\begin{table*}[t!]
\small
\begin{center}
% \setlength\tabcolsep{1pt}
\begin{tabular}{ccccccc}
\thickhline 
& & & \textsc{OnlySRC} & \textsc{OnlyTGT} & \textsc{Combine} & \textsc{EasyAdapt} \\ \hline
\multirow{4}{*}{\textsc{WLP}$\Rightarrow$\textsc{PubMedM\&M}} 
& \multirow{2}{*}{NER} & \textsc{BERT}     & 60.91$\pm$1.0 & 72.45$\pm$0.3 & 70.73$\pm$0.2 & \bf72.61$\pm$0.7 \\
&                      & \textsc{ProcBERT} & 63.65$\pm$0.5 & 74.55$\pm$0.2 & 73.96$\pm$0.4 & \bf74.77$\pm$0.4 \\
& \multirow{2}{*}{RE}  & \textsc{BERT}     & 73.09$\pm$0.6 & 77.54$\pm$0.8 & 79.02$\pm$0.3 & \bf79.99$\pm$0.6 \\ 
&                      & \textsc{ProcBERT} & 74.28$\pm$0.7 & 79.95$\pm$0.4 & 79.84$\pm$0.7 & \bf81.22$\pm$0.3 \\ \hline
\multirow{4}{*}{\textsc{ChemSyn}$\Rightarrow$\textsc{PubMedM\&M}} 
 & \multirow{2}{*}{NER} & \textsc{BERT}     & 65.27$\pm$0.7 & 72.45$\pm$0.3 & 72.91$\pm$0.5 & \bf72.91$\pm$0.4 \\
 &                      & \textsc{ProcBERT} & 68.04$\pm$0.5 & 74.55$\pm$0.2 & 75.14$\pm$0.3 & \bf75.16$\pm$0.2 \\
 & \multirow{2}{*}{RE}  & \textsc{BERT}     & 71.38$\pm$0.5 & 77.54$\pm$0.8 & 78.28$\pm$0.6 & \bf78.91$\pm$0.5 \\ 
&                      & \textsc{ProcBERT} & 73.61$\pm$0.7 & 79.95$\pm$0.4 & 80.30$\pm$0.7 & \bf80.47$\pm$0.6 \\ \hline
\multirow{4}{*}{\textsc{WLP}$\Rightarrow$\textsc{ChemSyn}} 
& \multirow{2}{*}{NER} & \textsc{BERT} \\
&                      & \textsc{ProcBERT} \\
& \multirow{2}{*}{RE} & \textsc{BERT} \\ 
& & \textsc{ProcBERT} \\ \hline
\multirow{4}{*}{\textsc{ChemSyn}$\Rightarrow$\textsc{WLP}} 
& \multirow{2}{*}{NER} & \textsc{BERT} \\
& & \textsc{ProcBERT} \\
& \multirow{2}{*}{RE} & \textsc{BERT} \\ 
& & \textsc{ProcBERT} \\ \hline
\thickhline 
\end{tabular}
\end{center}
\caption{\label{tab:sda_results}Results. }
\end{table*}
\end{comment}


% \subsection{In-domain Labeled Data}
\subsection{Budget-Aware Performance Comparison}
% \FB{This section motivates the need for our annotated datasets}
% Although pre-training a domain-specific langugae model from scratch leads to significant performance gains, one non-negligible down side is the prohibitive cost \citep{Strubell2019EnergyAP}. 
% As mentioned above, pre-training often comes with relatively large cost. 
% Therefore, one natural question is, given a specific budget, should we go straight into in-domain pre-training or simply annotate more training data on the target domain? 
% As realistically we only have limited budget, it is not clear whether we should go straight into in-domain pre-training or simply annotate more training data on the target domain? 
% \FB{Can we ask this question in the abstract or intro?} 
As we have shown the effectiveness of pre-training-based and supervised domain adaptation methods above, we now compare these two types of methods in a budget-aware setting to reveal their practical applicability. We use the pre-training of \textsc{ProcBERT-30k} and the annotation of \textsc{ChemSyn} for example.

\subsubsection{Cost Calculation}
To facilitate a budget-aware comparison, we first calculate the cost of each method here.

% \paragraph{\textsc{ChemSyn} Annotation}
\paragraph{\textsc{ChemSyn} Annotation}
For \textsc{ChemSyn}, there are in total 600 files, and each file has 6.87 sentences on average and takes around 14.33 minutes to annotate. Our annotators were payed 13 USD / hour. With double-annotating half of the files, the overall annotation expense for \textsc{ChemSyn} was roughly 2,800 USD.

\paragraph{\textsc{PubMedM\&M} Annotation}
For \textsc{PubMedM\&M}, there are in total 191 files, and each file has 7.90 sentences on average and takes around 16.47 minutes to annotate. Our annotators were payed 13 USD / hour. With double-annotating all 191 files, the overall annotation expense for \textsc{ChemSyn} was roughly 1,360 USD.

\paragraph{\textsc{ProcBERT} Pre-training} 
% \paragraph{\textsc{ProcBERT-30k} Pre-training} 
As introduced in Section \ref{sec:implement}, the whole training process of \textsc{ProcBERT} consists of two parts. In the first part, the model will be trained for 1 million steps with a rough speed of 4.71 step / second. In the second part, the model will be further trained on the longer input sequence for 100k steps with a speed of 1.83 step / second. Therefore, the overall training will take around
% (1000000/4.71+100000/1.83)/3600
74 hours. We use one on-demand TPU v3 with 8 cores from the Google Cloud Platform. Given the price on the official website\footnote{https://cloud.google.com/tpu/pricing} 8 USD / hour, the cost on TPU is around 590 USD. After including other expenses like data storage, the total cost for the pre-training is around 620 USD.


\subsubsection{Experiments}
% \FB{There should be a better way to present this section.} 
% As we can see that the cost of \textsc{ProcBERT-30k} pre-training almost equals to the annotation of 133 \textsc{ChemSyn} files. 
% Therefore, one experiment we can do is to compare \textsc{ProcBERT} with \textsc{BERT} while there are 133 more files (1/3 original training data) in the training set of \textsc{BERT} so that two models are compared equally cost-wise.
% Since we now know the cost of these two method, we want to see which direction gives us a better performance. 
% Since we now know the cost of these two methods, 
% what we need is a guidance of method selection, which can help make the most of the limited budget in practice. To figure this out, we compare these two methods in a budget-aware setting.
Assume we want to work on the \textsc{ChemSyn} dataset with NER and RE two tasks without any labeled training data.
As a first step, we train \textsc{BERT} on the \textsc{PubMedM\&M} dataset  because these two datasets are in close domains and have the same label space.
We use this result as a "cost-free" baseline to see how much a budget can improve the performance.
Then given a specific budget, we experiment with the two following strategies:

\paragraph{\textsc{BERT}} All the money is used to annotate the training data of \textsc{ChemSyn}, and the off-the-shelf domain-agnostic language model \textsc{BERT} is deployed for experiments.

\paragraph{\textsc{EasyAdapt}} Pass

\paragraph{\textsc{SciBERT}} Pass

\paragraph{\textsc{ProcBERT}} We prioritize the pre-training of \textsc{ProcBERT-30k} and use the rest of the money for \textsc{ChemSyn} annotation.

% \paragraph{\textsc{Proc-RoBERTa}} Pass




% And Our goal is to compare performance gains we can get from these two strategies over using out-of-domain \textsc{PubMedM\&M} for training.
The budgets of \textsc{BERT} and \textsc{EasyAdapt} start with 0 USD while the budget of \textsc{ProcBERT} starts with 620 USD. We increase them 155 USD each time until they reach a capacity of 1,850 USD, which is the annotation expense of the whole training set of \textsc{ChemSyn}
% where we use the "free" \textsc{PubMedM\&M} dataset for training because these two datasets are in close domains and have the same label space.
% We increase the budgets of two strategies 310 USD each time until they exceeds 1,850 USD, which is the annotation expense of the whole training set of \textsc{ChemSyn}. 


The development set performance gains of the two above strategies over the "cost-free" baseline (denoted as $\triangle F_1$) on NER and RE are presented in Figure \ref{fig:budget}.
% Note that when the budget is 620 USD, there is no annotated training set for \textsc{Pre-train}, so we use the training set of \textsc{PubMedM\&M} because these two datasets are in close domains and have the same label space.
% Specifically, what we do is to split the training data of \textsc{ChemSyn} into 6 equivalent subsets, and we compare the performance of \textsc{ProcBERT} trained on $n$ subsets with the performance of \textsc{BERT} trained on $(n+2)$ subsets to see which method works better. 
% The dev set results of the two above methods are shown in the Table \ref{tab:compare_results}. 
We can see that both \textsc{BERT} and \textsc{BERT} perform much better when the in-domain training set is available. \textsc{ProcBERT} does not work as well as \textsc{BERT} when the budget is lower mainly because it does not have enough in-domain training data. However, starting with a budget of 1240 USD, \textsc{ProcBERT} outperforms \textsc{BERT} demonstrating that we should consider the pre-training approach only if we are in high-resource scenarios.

\begin{comment}
\begin{table}[h!]
\small
\begin{center}
% \setlength\tabcolsep{3pt}
\scalebox{0.85}{
\begin{tabular}{ccccccc}
\thickhline  & \multicolumn{2}{c}{NER} &  \multicolumn{2}{c}{RE} \\ 
Budget & \textsc{Annotate} & \textsc{Pre-train} & \textsc{Annotate} & \textsc{Pre-train} \\ \hline
% 1 & 92.67$\pm$0.1 & 94.20$\pm$0.1 & 91.04$\pm$0.3 & 92.39$\pm$0.3 \\ 
% 2 & 94.53$\pm$0.1 & 95.56$\pm$0.2 & 92.15$\pm$0.4 & 93.67$\pm$0.1 \\ 
% 3 & 95.16$\pm$0.1 & 95.92$\pm$0.2 & 93.15$\pm$0.2 & 94.37$\pm$0.2 \\ 
% 4 & 95.37$\pm$0.1 & 95.97$\pm$0.1 & 93.17$\pm$0.5 & 94.52$\pm$0.2 \\ 
% 5 & 95.67$\pm$0.2 & 96.14$\pm$0.1 & 93.86$\pm$0.1 & 94.77$\pm$0.2 \\ 
% 6 & 95.81$\pm$0.1 & 96.36$\pm$0.2 & 93.91$\pm$0.3 & 94.95$\pm$0.2 \\ 
0   & 70.17$\pm$0.9 & - & 78.72$\pm$0.5 & - \\
310 & 92.67$\pm$0.1 & - & 91.04$\pm$0.3 & - \\
620 & \bf94.53$\pm$0.1 & 78.72$\pm$0.9 & \bf92.15$\pm$0.4 & 82.46$\pm$0.5 \\ 
930 & \bf95.16$\pm$0.1 & 94.20$\pm$0.1 & \bf93.15$\pm$0.2 & 92.39$\pm$0.3 \\ 
1240 & 95.37$\pm$0.1 & \bf95.56$\pm$0.2 & 93.17$\pm$0.5 & \bf93.67$\pm$0.1 \\ 
1550 & 95.67$\pm$0.2 & \bf95.92$\pm$0.2 & 93.86$\pm$0.1 & \bf94.37$\pm$0.2 \\ 
1850 & 95.81$\pm$0.1 & \bf95.97$\pm$0.1 & 93.91$\pm$0.3 & \bf94.52$\pm$0.2 \\ 
% 5 & - & 96.14$\pm$0.1 & - & 94.77$\pm$0.2 \\ 
% 6 & - & 96.36$\pm$0.2 & - & 94.95$\pm$0.2 \\ 
\thickhline
\end{tabular}
}
\end{center}
\caption{\label{tab:compare_results} Result. \FB{This table should be replaced with a figure.}}
\end{table}
\end{comment}



\begin{table*}[t!]
\small
\begin{center}
% \setlength\tabcolsep{1pt}
\resizebox{\textwidth}{!}{\begin{tabular}{ccccccc}
\thickhline 
& \multirow{2}{*}{Budget} & \multicolumn{4}{c}{Model (F1 / \# sent.)} \\ 
% &  &  & \textsc{BERT} (\$0) & \textsc{Proc-RoBERTa} (\$752) & \textsc{ProcBERT} (\$620) & \textsc{SciBERT} (\$1344) \\ \hline
&  &  \textsc{BERT} & \textsc{Proc-RoBERTa} & \textsc{ProcBERT} & \textsc{SciBERT} \\ 
&  &  (\$0) & (\$752) & (\$620) & (\$1344) \\ \hline

% \resizebox{\textwidth}{!}{\begin{tabular}{ccccccccccc}
% \thickhline 
% & \multirow{2}{*}{Budget} & \multicolumn{8}{c}{Model (F1 / \# sent.)} \\ 
% % &  &  \multicolumn{2}{c}{\textsc{BERT}(\$0)} & \multicolumn{2}{c}{\textsc{Proc-RoBERTa}(\$752)} & \multicolumn{2}{c}{\textsc{ProcBERT}(\$620)} & \multicolumn{2}{c}{\textsc{SciBERT}(\$1344)} \\
% &  &  \multicolumn{2}{c}{\textsc{BERT}} & \multicolumn{2}{c}{\textsc{Proc-RoBERTa}} & \multicolumn{2}{c}{\textsc{ProcBERT}} & \multicolumn{2}{c}{\textsc{SciBERT}} \\ 
% &  &  \multicolumn{2}{c}{(\$0)} & \multicolumn{2}{c}{(\$752)} & \multicolumn{2}{c}{(\$620)} & \multicolumn{2}{c}{(\$1344)} \\ 
% &  &  NER & RE & NER & RE & NER & RE & NER & RE \\ \hline

\multirow{3}{*}{\textsc{PubMedM\&M}$\Rightarrow$\textsc{ChemSyn}}  
 & \$600 & 70.0$\pm$0.0 F1 / 1000 & 70.0$\pm$0.0 F1 / 1000 & 70.0$\pm$0.0 F1 / 1000 & 70.0$\pm$0.0 F1 / 1000   \\ 
 & \$1500 \\ 
 & \$2500 \\ \hline
\multirow{3}{*}{\textsc{WLP}$\Rightarrow$\textsc{ChemSyn}} 
 & \$600 \\ 
 & \$1500 \\ 
 & \$2500 \\ \hline
\multirow{3}{*}{\textsc{WLP}$\Rightarrow$\textsc{PubMedM\&M}} 
 & \$600 \\ 
 & \$1500 \\ 
 & \$2500 \\ \hline
\multirow{3}{*}{\textsc{ChemSyn}$\Rightarrow$\textsc{PubMedM\&M}} 
 & \$600 \\ 
 & \$1500 \\ 
 & \$2500 \\ \hline
\multirow{3}{*}{\textsc{ChemSyn}$\Rightarrow$\textsc{WLP}} 
 & \$600 \\ 
 & \$1500 \\ 
 & \$2500 \\ \hline
\multirow{3}{*}{\textsc{PubMedM\&M}$\Rightarrow$\textsc{WLP}} 
 & \$600 \\ 
 & \$1500 \\ 
 & \$2500 \\ 
\thickhline 
\end{tabular}}
\end{center}
\caption{\label{tab:ner_results} NER Results. }
\end{table*}

\begin{table*}[t!]
\small
\begin{center}
% \setlength\tabcolsep{1pt}
\resizebox{\textwidth}{!}{\begin{tabular}{ccccccc}
\thickhline 
& \multirow{2}{*}{Budget} & \multicolumn{4}{c}{Model (F1 / \# sent.)} \\ 
% &  &  & \textsc{BERT} (\$0) & \textsc{Proc-RoBERTa} (\$752) & \textsc{ProcBERT} (\$620) & \textsc{SciBERT} (\$1344) \\ \hline
&  &  \textsc{BERT} & \textsc{Proc-RoBERTa} & \textsc{ProcBERT} & \textsc{SciBERT} \\ 
&  &  (\$0) & (\$752) & (\$620) & (\$1344) \\ \hline

\multirow{3}{*}{\textsc{PubMedM\&M}$\Rightarrow$\textsc{ChemSyn}}  
 & \$600 & 70.0$\pm$0.0 F1 / 1000 & 70.0$\pm$0.0 F1 / 1000 & 70.0$\pm$0.0 F1 / 1000 & 70.0$\pm$0.0 F1 / 1000   \\ 
 & \$1500 \\ 
 & \$2500 \\ \hline
\multirow{3}{*}{\textsc{WLP}$\Rightarrow$\textsc{ChemSyn}} 
 & \$600 \\ 
 & \$1500 \\ 
 & \$2500 \\ \hline
\multirow{3}{*}{\textsc{WLP}$\Rightarrow$\textsc{PubMedM\&M}} 
 & \$600 \\ 
 & \$1500 \\ 
 & \$2500 \\ \hline
\multirow{3}{*}{\textsc{ChemSyn}$\Rightarrow$\textsc{PubMedM\&M}} 
 & \$600 \\ 
 & \$1500 \\ 
 & \$2500 \\ \hline
\multirow{3}{*}{\textsc{ChemSyn}$\Rightarrow$\textsc{WLP}} 
 & \$600 \\ 
 & \$1500 \\ 
 & \$2500 \\ \hline
\multirow{3}{*}{\textsc{PubMedM\&M}$\Rightarrow$\textsc{WLP}} 
 & \$600 \\ 
 & \$1500 \\ 
 & \$2500 \\ 
\thickhline 
\end{tabular}}
\end{center}
\caption{\label{tab:re_results} RE Results. }
\end{table*}

==> sections_old/4_related.tex <==


\paragraph{Domain Adaptation via Pre-trained Language model}
There has been primarily two directions of using pre-trained language model for domain adaptation. The first direction is to pre-train a language model on the in-domain data from scratch \citep{Beltagy2019SciBERTAP, Huang2019ClinicalBERTMC, Nguyen2020BERTweetAP}, which requires to collect a huge amount of domain-specific data and is computationally expensive. The second one is to fine-tune the existing domain-general PLM like BERT or RoBERTa towards the target domain with the masked language model objective. This adaptation method could be domain-oriented \citep{Lee2020BioBERTAP, Gururangan2020DontSP} or task-oriented \citep{Logeswaran2019ZeroShotEL, Han2019UnsupervisedDA} depending on the specificity and size of the used corpus. Our work compares these two directions in the context of procedural text understanding on 6 related datasets, and shows that pre-training an in-domain language model from scratch works better empirically probably due to the in-domain vocabulary.

\paragraph{Supervised Domain Adaptation}
Supervised domain adaptation has been studied actively. One of the most influential approaches is \textsc{EasyAdapt} \citep{Daum2007FrustratinglyED}, which separates domain-specific and domain-general features via different feature spaces, and uses domain-general features for feature augmentation on the target domain. Many recent works employ this technique with the neural network. \citet{Kim2016FrustratinglyEN} deploys a shared and K private Bi-LSTM
encoders for feature extraction; \citet{Peng2017MultitaskDA} uses just one
representation learner but segments the generated hidden vector into multiple sub-vectors for different domains; \citet{Li2020SemisupervisedDA} uses the off-the-shelf BRET model for the contextual embedding and enforces the shared features to be domain-agnostic via an adversarial training loss. In contrast, our work focuses on exploring the importance of using different pre-trained language models for different domains and improves the shared features via a tunable hyper-parameter.

\paragraph{Procedural Text Understanding}
Procedural text is a genre of text describing how to fulfil a specific task. One line of work in this domain is to create new process-understanding datasets in different domains, e.g., entity tracking for scientific process \citep{Dalvi2018TrackingSC} and recipes \citep{Kiddon2016GloballyCT}, or information extraction for wet lab protocols \citep{Tabassum2020WNUT2020T1} and chemical patents \citep{Nguyen2020ChEMUNE}. Another line of work designs complicated neural network models based on the features of procedural text such as the structural constraints inherent in the processes \citep{Tandon2018ReasoningAA, Gupta2019TrackingDA}.
In our paper, we tackle the the procedural text understanding task from the perspective of domain adaptation (DA) as it is a special domain of text, and many successful DA techniques like in-domain language model pre-training (unsupervised) and feature augmentation (supervised) have not been fully explored.

==> sections_old/5_meature_utility.tex <==



\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=8cm]{figures/chemsyn_ner_budget.pdf}
        \caption{\pubmed{}$\Rightarrow$\chemsyn{}}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=8cm]{figures/wlp_ner_budget.pdf}
        \caption{\chemsyn{}$\Rightarrow$\wlp{}}
    \end{subfigure}
    \caption{\label{fig:budget} Comparison of two domain adaptation strategies: 1) \emojibert allocate all available funds to data annotation; 2)  \emojiprocbert pre-train \procbert{} on in-domain data, then use the remaining budget for annotation.  For small budgets, the former yields the best performance on  NER, but as the budget increases, the later becomes the best choice.}
\end{figure*}

Given the estimated unit cost of annotation $C_a$ (\S\ref{sec:estimate_c_a}) and pre-training $C_p$ (\S\ref{sec:estimate_c_p}), we now evaluate the utility (i.e., adapted model's performance) of combining annotation and pre-training $U(X_a, X_p)$ to find an optimal strategy for domain adaptation under fixed budget constraints $X_a C_a + X_p C_P \leq B$. $X_a$ is the number of annotated documents and $X_p$ is the number of TPU hours needed for pre-training.    
%In this section, we first introduce the two involved tasks in \S\ref{sec:utility_task}. Then we describe how we use labeled data from both source and target domains via the supervised domain adaptation framework \easyadapt{} in \S\ref{sec:utility_easy}. Lastly, we show our experimental setup for the utility measurement (\S\ref{sec:utility_setup}) and give a detailed analysis of the measured utilities under different budgets (\S\ref{sec:utility_result}).



%        under a constrained budget.  For budgets less than \$1,000 
%    \bertbase{} and \procbert{} on NER (dev set) under two domain adaptation settings \pubmed{}$\Rightarrow$\chemsyn{} (a) and \chemsyn{}$\Rightarrow$\wlp{} (b). 
% The budget of each strategy starts with the pre-training cost of its in-domain language model, and
% We gradually increase the budget of each strategy (155 USD each time) until its annotation portion reaches the expense of the training set of the target domain dataset.


\subsection{NLP Tasks and Models}
\label{sec:utility_task}
We experiment with two NLP tasks, Named Entity Recognition (NER) and Relation Extraction (RE), for comparing domain adaptation strategies under varied budgets. 
% NER is a sequence labeling task where the model detects named entity spans. RE is a classification task where the model predicts the relation between two entities in the same sentence. 
%We use a different fine-tuning architecture for each task. 
For NER, we follow \citet{devlin-etal-2019-bert} to feed the contextualized embedding of each token into a linear classification layer with softmax output. 
% For RE, our architecture is similar to \citet{Soares2019MatchingTB}, where four special tokens \texttt{[E1]}, \texttt{[\textbackslash E1]}, \texttt{[E2]}, \texttt{[\textbackslash E2]} are used to specify the positions of two entities, and the contextualized embeddings of \texttt{[E1]} and \texttt{[E2]} are concatenated as input to a final linear layer that is used to predict the relation.
For RE, we use the state-of-the-art architecture following \citep{Zhong2020AFE, tamari-etal-2021-process-level}, where four special tokens are inserted to specify the positions and types of entities in a pre-trained sentence encoder. 
%For example, \texttt{[E1-PER]}, \texttt{[\textbackslash E1-PER]}, \texttt{[E2-LOC]}, and \texttt{[\textbackslash E2-LOC]} are used to denote the spans of an entity pair with \texttt{PERSON} and \texttt{LOCATION} types. Then, the contextualized representations of \texttt{[E1-PER]} and \texttt{[E2-LOC]} are concatenated as input to a final linear layer to predict the relation. We used F\textsubscript{1} score as the evaluation metric for both tasks. An NER prediction is considered correct only if its label and boundary both match with the gold entity mention.
% , and we use the Perl script \texttt{conlleval}\footnote{\url{https://www.clips.uantwerpen.be/conll2000/chunking/output.html}} for evaluation. 
For RE, the input is the gold entity mentions, and a relation prediction is correct when its label matches with the gold relation. 


\subsection{Budget-constrained Experimental Setup}
\label{sec:utility_setup}

As we have three procedural text datasets (\S \ref{sec:estimate_c_a}) annotated with entities and relations, we can experiment with six different source and target domain combinations. For each (Source $\Rightarrow$ Target) pair, we compare five different pre-trained language models when adapted to the procedural text domain under varying budgets.

Based on the estimations of the annotation cost $C_a$ (\S\ref{sec:estimate_c_a}) and pre-training cost $C_p$ (\S\ref{sec:estimate_c_p}), we conduct the budget-constrained domain adaptation experiment. For example, if we have \$1,500 and the \pubmed{} corpus, to build a NER model that works best for the \chemsyn{} domain (\textsc{\pubmed{}}$\Rightarrow$\textsc{ChemSyn}), we can spend all \$1,500 to annotate 2500 sentences from the \textsc{ChemSyn} domain to fine-tune off-the-shelf BERT. Or alternatively, we could first spend \$800 to pre-train Proc-RoBERTa, then fine-tune it on 1155 sentences annotated in the \textsc{ChemSyn} domain using the remaining of \$700. Under both budgeting strategies, an additional experiment is performed to choose one of two domain adaption methods that maximizes performance: 1) a model that simply uses the annotated data in the target domain for fine-tuning; or 2) a model which is fine-tuned using a variant of \easyadapt{} \citep{Daum2007FrustratinglyED} to leverage annotated data in both the source and target domains (see below for details). We select the approach that has better development set performance and report its test set result in Table \ref{tab:ner_results} and \ref{tab:re_results} (see Appendix \ref{sec:hyper_para} for more details about hyper-parameters).  




%We found that including source domain data does not help in every case, therefore we evaluate two models: 1) a model that uses \easyadapt{} to leverage available data from both domains; 2) a model that only uses the target domain data for fine-tuning. Then we select the model that has better development set performance and report its test set result.  

%Results that were obtained using \easyadapt{} are marked with ``\textdagger'' in Tables \ref{tab:ner_results} and \ref{tab:re_results}.
%We report averages across five random seeds, with standard deviations as subscripts.





%As in a real-world scenario, an NLP practitioner has two main strategies to choose from: (1) spend all the budget on annotating task-specific data to fine-tune the generic BERT model; or (2) pre-train a new in-domain language model, then use the remaining budget to obtain some annotated data.





%In a real-world scenario to optimize the NER/RE model performance, an NLP practitioner can either choose to


%to imitate the real-world situations, in which different NLP practitioners may have different amounts of resources. 
% Given a budget constraint and pre-trained model, we calculate remaining funds for data annotation after factoring in pre-training cost (calculated in \S\ref{sec:pre-training_cost}). Then we use the remaining budget to ``purchase'' target domain data, considering the price (\$ / sent.) listed in Table \ref{tab:task_statistics}.
%For instance, if the remaining budget is able to buy $N$ annotated sentences, we will take the first $N$ sentences from a set of ordered files, and truncate the last selected file to have exactly $N$ sentences when necessary.
% If the pre-training cost goes over the total budget, or available data goes under the annotation budget, we leave the result as \quotes{NA}.
%Once we have the target domain training data ready, 






%The main reason for creating the second model is that \easyadapt{} is more effective in low-resource scenarios where the annotated target corpus is smaller. However, the annotated target dataset in some of the combination strategies is larger. In this case, utilizing the source domain data (with \easyadapt{}) can hurt the performance because there is already sufficient data in the target domain to learn an efficient model.

% For \pubmed{} and \chemsyn{}, we use the original data split for the domain adaptation experiments.
% For \wlp{} \citep{Tabassum2020WNUT2020T1}, the dataset is split into four subsets randomly: train, dev, test, and test-2020, and we follow the setup of the top-performing system \textsc{mgsohrab} \citep{Sohrab2020mgsohrabAW} in the EMNLP 2020 WNUT shared task, to merge the original train and dev as the new train set, and treat test and test-2020 as the new dev and test set respectively. 
% The data spilt of three datasets can be found in Table \ref{tab:sda_stats}.

% We follow the experimental setup of the respective paper for each task, and report averages and standard deviations across five random seeds for all our experiments. 
 


\begin{table*}[t!]
\small
\begin{center}
\resizebox{\textwidth}{!}{\begin{tabular}{ccC{0.8cm}C{0.8cm}C{0.8cm}C{0.8cm}C{0.8cm}C{0.8cm}C{0.8cm}C{0.8cm}C{0.8cm}C{0.8cm}C{0.8cm}C{0.8cm}}
% \resizebox{\textwidth}{!}{\begin{tabular}{cccHcccc}

\toprule 

& &  \multicolumn{2}{c}{\textbf{\bertbase{}}} & \multicolumn{2}{c}{\textbf{\bertlarge{}}} & \multicolumn{2}{c}{\textbf{\procbert{}}} & \multicolumn{2}{c}{\textbf{\procroberta{}}} & \multicolumn{2}{c}{\textbf{\scibert{}}} \\ 
\multirow{2}{*}{\textbf{Source $\Rightarrow$ Target Domain}} & \multirow{2}{*}{\textbf{Budget}} & \multicolumn{2}{c}{\$0} & \multicolumn{2}{c}{\$0} & \multicolumn{2}{c}{\$620} & \multicolumn{2}{c}{\$800} & \multicolumn{2}{c}{\$1340} \\ \cmidrule(l){3-4}\cmidrule(l){5-6}\cmidrule(l){7-8}\cmidrule(l){9-10} \cmidrule(l){11-12}

&  & F\textsubscript{1} & (\#sent) & F\textsubscript{1} & (\#sent)  & F\textsubscript{1} & (\#sent)  & F\textsubscript{1} & (\#sent)  & F\textsubscript{1} & (\#sent) \\
\midrule
\multirow{3}{*}{\textsc{PubMedM\&M}$\Rightarrow$\textsc{ChemSyn}}  
 & \$700  & 92.58\textsubscript{0.2} & (1166) & \textbf{93.32}\textsubscript{0.2}\textsuperscript{\textdagger} & (1166) & 90.96\textsubscript{0.4}\textsuperscript{\textdagger} & (133) & \multicolumn{2}{c}{NA} & \multicolumn{2}{c}{NA} \\ 
 & \$1500 & 93.32\textsubscript{0.2} & (2500)  & 93.94\textsubscript{0.4}\textsuperscript{\textdagger} & (2500) & \textbf{94.68}\textsubscript{0.2} & (1466)  & 93.60\textsubscript{0.3}\textsuperscript{\textdagger} & (1166) & 92.44\textsubscript{0.3}\textsuperscript{\textdagger} & (266)  \\ 
 & \$2300 & 94.49\textsubscript{0.2} & (3833)  & 94.79\textsubscript{0.2} & (3833)  & \textbf{95.11}\textsubscript{0.2} & (2800)  & 94.89\textsubscript{0.2} & (2500)  & 94.22\textsubscript{0.2} & (1600)  \\  \midrule
 
\multirow{3}{*}{\textsc{WLP}$\Rightarrow$\textsc{ChemSyn}} 
 & \$700  & 92.94\textsubscript{0.2}\textsuperscript{\textdagger} & (1166) & \textbf{93.06}\textsubscript{0.1}\textsuperscript{\textdagger} & (1166) & 90.40\textsubscript{0.3}\textsuperscript{\textdagger} & (133) & \multicolumn{2}{c}{NA} & \multicolumn{2}{c}{NA} \\ 
 & \$1500 & 93.32\textsubscript{0.2} & (2500)  & 94.23\textsubscript{0.1}\textsuperscript{\textdagger} & (2500)  & \textbf{94.73}\textsubscript{0.2}\textsuperscript{\textdagger} & (1466)  & 94.19\textsubscript{0.1}\textsuperscript{\textdagger} & (1166)  & 92.09\textsubscript{0.3}\textsuperscript{\textdagger} & (266) \\
 & \$2300 & 94.49\textsubscript{0.2} & (3833)  & 94.79\textsubscript{0.3}\textsuperscript{\textdagger} & (3833)  & \textbf{95.37}\textsubscript{0.1}\textsuperscript{\textdagger} & (2800)  & 94.82\textsubscript{0.4}\textsuperscript{\textdagger} & (2500)  & 94.22\textsubscript{0.2} & (1600) \\ \midrule
 
\multirow{2}{*}{\textsc{WLP}$\Rightarrow$\textsc{PubMedM\&M}} 
 & \$700 & 71.88\textsubscript{0.4} & (686)  & \textbf{72.93}\textsubscript{0.5}\textsuperscript{\textdagger} & (686)  & 63.80\textsubscript{0.7}\textsuperscript{\textdagger} & (78)  & \multicolumn{2}{c}{NA}  & \multicolumn{2}{c}{NA} \\
 & \$1500 & \multicolumn{2}{c}{NA}  & \multicolumn{2}{c}{NA}  & \textbf{74.57}\textsubscript{0.3}\textsuperscript{\textdagger} & (862)  & 73.75\textsubscript{0.1} & (686)  & 69.94\textsubscript{0.4}\textsuperscript{\textdagger} & (156) \\
%  & \$2300 & \multicolumn{2}{c}{NA}  & \multicolumn{2}{c}{NA}  & \multicolumn{2}{c}{NA}  & \multicolumn{2}{c}{NA}  & \multicolumn{2}{c}{NA} \\  
 \midrule
 
\multirow{2}{*}{\textsc{ChemSyn}$\Rightarrow$\textsc{PubMedM\&M}} 
 & \$700 & 73.14\textsubscript{0.5}\textsuperscript{\textdagger} & (686)  & \textbf{74.24}\textsubscript{0.6}\textsuperscript{\textdagger} & (686)  & 71.16\textsubscript{0.4}\textsuperscript{\textdagger} & (78)  & \multicolumn{2}{c}{NA}  & \multicolumn{2}{c}{NA} \\
 & \$1500 & \multicolumn{2}{c}{NA}  & \multicolumn{2}{c}{NA}  & \textbf{75.81}\textsubscript{0.7}\textsuperscript{\textdagger} & (862)  & 74.78\textsubscript{0.4}\textsuperscript{\textdagger} & (686)  & 72.87\textsubscript{0.3}\textsuperscript{\textdagger} & (156) \\
%  & \$2300 & \multicolumn{2}{c}{NA}  & \multicolumn{2}{c}{NA}  & \multicolumn{2}{c}{NA}  & \multicolumn{2}{c}{NA}  & \multicolumn{2}{c}{NA} \\ 
 \midrule
 
\multirow{3}{*}{\textsc{ChemSyn}$\Rightarrow$\textsc{WLP}} 
 & \$700 & 72.91\textsubscript{0.3}\textsuperscript{\textdagger} & (1590)  & \textbf{73.30}\textsubscript{0.3}\textsuperscript{\textdagger} & (1590)  & 72.69\textsubscript{0.2}\textsuperscript{\textdagger} & (181)  & \multicolumn{2}{c}{NA}  & \multicolumn{2}{c}{NA} \\
 & \$1500 & 73.69\textsubscript{0.1}\textsuperscript{\textdagger} & (3409)  & 73.88\textsubscript{0.6}\textsuperscript{\textdagger} & (3409)  & \textbf{75.21}\textsubscript{0.2}\textsuperscript{\textdagger} & (2000)  & 74.24\textsubscript{0.3}\textsuperscript{\textdagger} & (1590)  & 72.52\textsubscript{0.9}\textsuperscript{\textdagger} & (363) \\
 & \$2300 & 73.85\textsubscript{0.4}\textsuperscript{\textdagger} & (5227)  & 74.23\textsubscript{0.5}\textsuperscript{\textdagger} & (5227)  & \textbf{75.51}\textsubscript{0.4}\textsuperscript{\textdagger} & (3818)  & 74.76\textsubscript{0.3}\textsuperscript{\textdagger} & (3409)  & 74.78\textsubscript{0.5}\textsuperscript{\textdagger} & (2181) \\  \midrule
 
\multirow{3}{*}{\textsc{PubMedM\&M}$\Rightarrow$\textsc{WLP}} 
 & \$700 & 73.21\textsubscript{0.1}\textsuperscript{\textdagger} & (1590)  & \textbf{73.43}\textsubscript{0.3}\textsuperscript{\textdagger} & (1590)  & 72.85\textsubscript{0.1}\textsuperscript{\textdagger} & (181)  & \multicolumn{2}{c}{NA}  & \multicolumn{2}{c}{NA} \\
 & \$1500 & 73.78\textsubscript{0.3}\textsuperscript{\textdagger} & (3409)  & 74.18\textsubscript{0.4}\textsuperscript{\textdagger} & (3409)  & \textbf{75.36}\textsubscript{0.1}\textsuperscript{\textdagger} & (2000)  & 73.93\textsubscript{0.3}\textsuperscript{\textdagger} & (1590)  & 72.89\textsubscript{0.3}\textsuperscript{\textdagger} & (363) \\
 & \$2300 & 74.09\textsubscript{0.2}\textsuperscript{\textdagger} & (5227)  & 74.32\textsubscript{0.3}\textsuperscript{\textdagger} & (5227)  & \textbf{75.73}\textsubscript{0.3}\textsuperscript{\textdagger} & (3818)  & 75.08\textsubscript{0.3}\textsuperscript{\textdagger} & (3409)  & 74.72\textsubscript{0.3}\textsuperscript{\textdagger} & (2181) \\  \bottomrule 
\end{tabular}}
\end{center}
\caption{\label{tab:ner_results} Experiment results for Named Entity Recognition (NER). With higher budgets (\$1500 and \$2300), our in-domain pre-training of \procbert{} achieves the best results in combination with data annotation. For a smaller budget (\$700), investing all funds in annotation and fine-tuning the standard \bertbase{} and \bertlarge{} (considered as cost-free) will yield the best outcome. \textbf{\#sent} is the number of sentences from the target domain, annotated under the given budget, used for training. \textsuperscript{\textdagger} indicates results using EasyAdapt (\S \ref{sec:utility_easy}), where source domain data helps. }
\end{table*}



\subsection{\easyadapt{}}
\label{sec:utility_easy}
In most of our experiments, 
% in a supervised learning setting, 
we have access to a relatively large amount of labeled data from a source domain, and varying amounts of data from the target domain. Instead of simply concatenating the source and target datasets for fine-tuning, we propose a simple, yet novel variation of EasyAdapt \citep{Daum2007FrustratinglyED} for pre-trained Transformers. More specifically, we create three copies of the model's contextualized representations: one represents the source domain, one represents the target, and the third is a domain-independent representation. These contextualized vectors are then concatenated and fed into a linear layer that is 3 times as large as the base model's.  When encoding data from a specific domain (e.g. \chemsyn{}), the other domain's representations are zeroed out (1/3 of the new representations will always be 0.0). This enables the domain-specific block of the linear layer to encode information specific to that domain, while the domain-independent parameters can learn to represent information that transfers across domains. This is similar to prior work on neural EasyAdapt \citep{kim2016frustratingly} for LSTMs.

\begin{comment}
two labeled corpora from source and target domains, and we want to use both corpora to achieve the best target domain performance.
We use a simple but effective feature augmentation framework \easyadapt{} \citep{Daum2007FrustratinglyED}, which sets up a distinct feature space for each domain, in addition to a shared feature representation.

% We now describe how our proposed method is applied to NER and RE two tasks.
The first step is to generate the feature representation of the input sequence.
In this case, for NER, it is the hidden vector generated from the last layer of the pre-trained language model for each word. For RE, it is the concatenation of contextual embeddings of special tokens \texttt{[E1]} and \texttt{[E2]} as introduced in \S\ref{sec:utility_task}.
Once we have the feature vector, 
% in \easyadapt{} is to build an augmented feature space.
% Suppose we have one source domain and one target domain, 
we replicate it three times,
% to build the augmented feature representation, 
where the first two vectors represent the source and target domain respectively, and the last vector represents the shared feature space.
Given a data point from one specific domain (source or target), 
% we concatenate the feature vector of its own domain and the feature vector of the shared domain.
% The concatenated vector is used as the final representation as well as the input to a linear classification layer for NER and RE.
we concatenate the feature vector of its own domain and the feature vector of the shared domain as the final feature representation.
In this last step, the feature representation is used as the input for a linear classification layer for NER and RE. 
%This linear classification layer is created by concatenating two linear layers corresponding to the two selected feature vectors.
\end{comment}

%For all six domain adaptation settings, the cost-free language models (\bertbase{} and \bertlarge{}) work better than in-domain language models when the budget is 700 USD, showing the effectiveness of data annotation in low-resource scenarios. 
% As the budget increases, the benefits of adding more labeled training data diminishes for cost-free language models, and in-domain language models start to take the lead. 
%Our language model \procbert{}, which is pre-trained from scratch on the self-collected procedural corpus while costing only 620 USD, performs the best at the budgets 1500 USD and 2300 USD, demonstrates that domain-specific pre-training will be more beneficial in high-resource settings. 


% \begin{table*}[t!]
% \small
% \begin{center}
% % \setlength\tabcolsep{1pt}
% \resizebox{\textwidth}{!}{\begin{tabular}{cccccccc}
% % \resizebox{\textwidth}{!}{\begin{tabular}{cccHcccc}
% \thickhline 
% & \multirow{2}{*}{Budget} & \multicolumn{5}{c}{Model} \\ 
% & &  \bertbase{} & \bertlarge{} & \procbert{} & \procroberta{} & \scibert{} \\ 
% &  &  (\$0) & (\$0) & (\$620) & (\$800) & (\$1340) \\ \hline
% \multirow{3}{*}{\textsc{PubMedM\&M}$\Rightarrow$\textsc{ChemSyn}}  
%  & \$700  & \textit{90.12$\pm$0.4} 1166  & 00.00$\pm$0.0 / 1166  & \textit{88.21$\pm$0.6} / 133   & NA                            & NA \\ 
%  & \$1500 & \textit{91.30$\pm$0.2} / 2500  & 00.00$\pm$0.0 / 2500  & \textit{92.06$\pm$0.4} / 1466  & \textit{91.25$\pm$0.7} / 1166  & \textit{89.58$\pm$0.5} / 266  \\ 
%  & \$2300 & 00.00$\pm$0.0 / 3833  & 00.00$\pm$0.0 / 3833  & \textit{92.57$\pm$0.2} / 2800  & \textit{92.07$\pm$0.3} / 2500  & \textit{91.55$\pm$0.2} / 1600  \\  \hline
 
% \multirow{3}{*}{\textsc{WLP}$\Rightarrow$\textsc{ChemSyn}} 
%  & \$700  & \textit{90.20$\pm$0.7} / 1166  & 00.00$\pm$0.0 / 1166  & \textit{88.01$\pm$0.6} / 133   & NA                            & NA \\ 
%  & \$1500 & \textit{91.34$\pm$0.3} / 2500  & 00.00$\pm$0.0 / 2500  & \textit{92.27$\pm$0.2} / 1466  & \textit{91.77$\pm$0.2} / 1166  & \textit{89.16$\pm$0.7} / 266  \\ 
%  & \$2300 & 00.00$\pm$0.0 / 3833  & 00.00$\pm$0.0 / 3833  & 00.00$\pm$0.0 / 2800  & 00.00$\pm$0.0 / 2500  & \textit{91.42$\pm$0.4} / 1600  \\  \hline
 
% \multirow{3}{*}{\textsc{WLP}$\Rightarrow$\textsc{PubMedM\&M}} 
%  & \$700  & 00.00$\pm$0.0 / 686   & 00.00$\pm$0.0 / 686   & \textit{74.63$\pm$0.4} / 78    & NA                            & NA \\ 
%  & \$1500 & NA                         & NA                         & \textit{80.10$\pm$0.6} / 862   & \textit{79.33$\pm$1.3} / 686  & \textit{75.70$\pm$1.1} / 156  \\ 
%  & \$2300 & NA                         & NA                         & NA                         & NA                            & NA \\  \hline
 
% \multirow{3}{*}{\textsc{ChemSyn}$\Rightarrow$\textsc{PubMedM\&M}} 
%  & \$700  & 00.00$\pm$0.0 / 686   & 00.00$\pm$0.0 / 686   & 00.00$\pm$0.0 / 78    & NA                            & NA \\ 
%  & \$1500 & NA                         & NA                         & 00.00$\pm$0.0 / 862   & 00.00$\pm$0.0 / 686  & 00.00$\pm$0.0 / 156  \\ 
%  & \$2300 & NA                         & NA                         & NA                         & NA                            & NA \\  \hline
 
% \multirow{3}{*}{\textsc{ChemSyn}$\Rightarrow$\textsc{WLP}} 
%  & \$700  & 00.00$\pm$0.0 / 1590  & 00.00$\pm$0.0 / 1590  & 00.00$\pm$0.0 / 181   & NA                            & NA \\ 
%  & \$1500 & 00.00$\pm$0.0 / 3409  & 00.00$\pm$0.0 / 3409  & 00.00$\pm$0.0 / 2000  & 00.00$\pm$0.0 / 1590  & 00.00$\pm$0.0 / 363  \\ 
%  & \$2300 & 00.00$\pm$0.0 / 5227  & 00.00$\pm$0.0 / 5227  & 00.00$\pm$0.0 / 3818  & 00.00$\pm$0.0 / 3409  & 00.00$\pm$0.0 / 2181  \\  \hline
 
% \multirow{3}{*}{\textsc{PubMedM\&M}$\Rightarrow$\textsc{WLP}} 
%  & \$700  & 00.00$\pm$0.0 / 1590  & 00.00$\pm$0.0 / 1590  & \textit{77.98$\pm$0.8} / 181   & NA                            & NA \\ 
%  & \$1500 & \textit{79.40$\pm$0.6} / 3409  & 00.00$\pm$0.0 / 3409  & \textit{80.45$\pm$0.2} / 2000  & \textit{78.79$\pm$1.1} / 1590  & \textit{78.76$\pm$0.5} / 363  \\ 
%  & \$2300 & \textit{79.93$\pm$0.5} / 5227  & 00.00$\pm$0.0 / 5227  & \textit{80.85$\pm$0.6} / 3818  & \textit{79.49$\pm$0.7} / 3409  & \textit{80.33$\pm$0.3} / 2181  \\  
% \thickhline 
% \end{tabular}}
% \end{center}
% \caption{\label{tab:re_results} RE Results (F\textsubscript{1} / \#Target Sentences).}
% \end{table*}


\subsection{Experimental Results and Analysis}
\label{sec:utility_result}

We present the test set NER and RE results with five annotation and pre-training combination strategies under six domain adaptation settings in Table \ref{tab:ner_results} and \ref{tab:re_results}, respectively. We report averages across five random seeds with standard deviations as subscripts. If the pre-training cost goes over the total budget, or available data goes under the annotation budget, we leave the result as \quotes{NA}.  We now discuss a set of key questions regarding pre-training-based domain adaptation under a constrained budget, which our experiments can shed some light on.

\paragraph{Should we prioritize pre-training or data annotation for domain adaptation?} For all six domain adaptation settings in Table \ref{tab:ner_results}, spending the entire budget on annotation and using off-the-shelf language models (\bertbase{} and \bertlarge{}) works the best for NER when the budget is 700 USD, showing the effectiveness of data annotation in low-resource scenarios. 
%Using a larger model like \bertlarge{} can boost the performance.
As the budget increases, performance gains from labelling additional data diminish, and pre-training in-domain language models takes the lead.
% the benefits of in-domain pre-training starts to outweigh adding cost-equivalent in-domain labeled data. 
\procbert{}, which is pre-trained from scratch on the {\sc Procedure+} corpus costing only 620 USD, performs best at budgets of 1500 and 2300 USD. 
This demonstrates that combining domain-specific pre-training with data annotation is the best strategy in high-resource settings.
%, where there is a reasonably large labeled dataset for in-domain models to learn task-specific knowledge. Note that the advantage of \procbert{} over other in-domain language models in this budget-aware comparison partially comes from the fact that it has more labeled training data due to its lower pre-training cost.Therefore, we compare all involved models in the same experimental setting in \S\ref{sec:other_procedural} to see how useful our procedural text-specific pre-training is for downstream tasks.
Similarly for RE, as shown in Table \ref{tab:re_results}, using all funds for data annotation and working with off-the-shelf models achieves better performance at lower budgets, while domain-specific pre-training starts to excel as the budget increases past a certain point.
% However, one thing we notice is that when the target domain dataset is \wlp{}, our in-domain language model \procbert{} can perform on par or even better than \bertbase{} at the budget of 700 USD. There are two reasons for this result: 1) The cost of per sentence annotation for \wlp{} is less than the cost of the other two datasets (Table \ref{tab:task_statistics}), which gives us more in-domain labeled data compared to the other two datasets with the same budget; 2) Using \easyadapt{} to take advantage of labeled data from other domains can alleviate the shortage of in-domain labeled data. This means, in practice, if we can find existing labeled data from domains close to our target domain, we can spend more money on the domain-specific pre-training over data annotation.


\begin{table*}[t!]
\small
\begin{center}
\resizebox{\textwidth}{!}{\begin{tabular}{ccC{0.8cm}C{0.8cm}C{0.8cm}C{0.8cm}C{0.8cm}C{0.8cm}C{0.8cm}C{0.8cm}C{0.8cm}C{0.8cm}C{0.8cm}C{0.8cm}}
% \resizebox{\textwidth}{!}{\begin{tabular}{cccHcccc}

\toprule 

& &  \multicolumn{2}{c}{\textbf{\bertbase{}}} & \multicolumn{2}{c}{\textbf{\bertlarge{}}} & \multicolumn{2}{c}{\textbf{\procbert{}}} & \multicolumn{2}{c}{\textbf{\procroberta{}}} & \multicolumn{2}{c}{\textbf{\scibert{}}} \\ 
\multirow{2}{*}{\textbf{Source $\Rightarrow$ Target Domain}} & \multirow{2}{*}{\textbf{Budget}} & \multicolumn{2}{c}{\$0} & \multicolumn{2}{c}{\$0} & \multicolumn{2}{c}{\$620} & \multicolumn{2}{c}{\$800} & \multicolumn{2}{c}{\$1340} \\ \cmidrule(l){3-4}\cmidrule(l){5-6}\cmidrule(l){7-8}\cmidrule(l){9-10} \cmidrule(l){11-12}

&  & F\textsubscript{1} & (\#sent) & F\textsubscript{1} & (\#sent)  & F\textsubscript{1} & (\#sent)  & F\textsubscript{1} & (\#sent)  & F\textsubscript{1} & (\#sent) \\
\midrule
\multirow{3}{*}{\textsc{PubMedM\&M}$\Rightarrow$\textsc{ChemSyn}}  
 & \$700  & 90.12\textsubscript{0.4}\textsuperscript{\textdagger} & (1166) & \textbf{90.71}\textsubscript{0.8}\textsuperscript{\textdagger} & (1166) & 88.21\textsubscript{0.6}\textsuperscript{\textdagger} & (133) & \multicolumn{2}{c}{NA} & \multicolumn{2}{c}{NA}\\ 
 & \$1500 & 91.30\textsubscript{0.2}\textsuperscript{\textdagger} & (2500) & 91.84\textsubscript{0.5}\textsuperscript{\textdagger} & (2500) & \textbf{92.06}\textsubscript{0.4}\textsuperscript{\textdagger} & (1466) & 91.25\textsubscript{0.7}\textsuperscript{\textdagger} & (1166) & 89.58\textsubscript{0.5}\textsuperscript{\textdagger} & (266) \\ 
 & \$2300 & 91.81\textsubscript{0.2}\textsuperscript{\textdagger} & (3833) & \textbf{92.90}\textsubscript{0.4}\textsuperscript{\textdagger} & (3833) & 92.57\textsubscript{0.2}\textsuperscript{\textdagger} & (2800) & 92.07\textsubscript{0.3}\textsuperscript{\textdagger} & (2500) & 91.55\textsubscript{0.2}\textsuperscript{\textdagger} & (1600) \\  \midrule
 
\multirow{3}{*}{\textsc{WLP}$\Rightarrow$\textsc{ChemSyn}} 
 & \$700  & \textbf{90.20}\textsubscript{0.7}\textsuperscript{\textdagger} & (1166) & 90.15\textsubscript{0.9} & (1166) & 88.01\textsubscript{0.6}\textsuperscript{\textdagger} & (133) & \multicolumn{2}{c}{NA} & \multicolumn{2}{c}{NA}\\ 
 & \$1500 & 91.34\textsubscript{0.3}\textsuperscript{\textdagger} & (2500) & 91.61\textsubscript{0.5}\textsuperscript{\textdagger} & (2500) & \textbf{92.27}\textsubscript{0.2}\textsuperscript{\textdagger} & (1466) & 91.77\textsubscript{0.2}\textsuperscript{\textdagger} & (1166) & 89.16\textsubscript{0.7}\textsuperscript{\textdagger} & (266) \\ 
 & \$2300 & 92.08\textsubscript{0.4}\textsuperscript{\textdagger} & (3833) & 92.73\textsubscript{0.4}\textsuperscript{\textdagger} & (3833) & \textbf{92.85}\textsubscript{0.2}\textsuperscript{\textdagger} & (2800) & 92.44\textsubscript{0.6}\textsuperscript{\textdagger} & (2500) & 91.42\textsubscript{0.4}\textsuperscript{\textdagger} & (1600) \\  \midrule
 
\multirow{2}{*}{\textsc{WLP}$\Rightarrow$\textsc{PubMedM\&M}} 
 & \$700 & 77.74\textsubscript{0.7}\textsuperscript{\textdagger} & (686) & \textbf{79.33}\textsubscript{1.3}\textsuperscript{\textdagger} & (686) & 74.63\textsubscript{0.4}\textsuperscript{\textdagger} & (78) & \multicolumn{2}{c}{NA} & \multicolumn{2}{c}{NA} \\ 
 & \$1500 & \multicolumn{2}{c}{NA} & \multicolumn{2}{c}{NA} & \textbf{80.10}\textsubscript{0.6}\textsuperscript{\textdagger} & (862) & 79.33\textsubscript{1.3}\textsuperscript{\textdagger} & (686) & 75.70\textsubscript{1.1}\textsuperscript{\textdagger} & (156) \\ 
%  & \$2300 & \multicolumn{2}{c}{NA} & \multicolumn{2}{c}{NA} & \multicolumn{2}{c}{NA} & \multicolumn{2}{c}{NA} & \multicolumn{2}{c}{NA} \\  
 \midrule
 
\multirow{2}{*}{\textsc{ChemSyn}$\Rightarrow$\textsc{PubMedM\&M}} 
 & \$700 & 77.02\textsubscript{0.6}\textsuperscript{\textdagger} & (686) & \textbf{77.31}\textsubscript{0.4}\textsuperscript{\textdagger} & (686) & 73.92\textsubscript{0.8}\textsuperscript{\textdagger} & (78) & \multicolumn{2}{c}{NA} & \multicolumn{2}{c}{NA} \\ 
 & \$1500 & \multicolumn{2}{c}{NA} & \multicolumn{2}{c}{NA} & \textbf{79.50}\textsubscript{0.7}\textsuperscript{\textdagger} & (862) & 77.12\textsubscript{1.2}\textsuperscript{\textdagger} & (686) & 75.43\textsubscript{0.6}\textsuperscript{\textdagger} & (156) \\ 
%  & \$2300 & \multicolumn{2}{c}{NA} & \multicolumn{2}{c}{NA} & \multicolumn{2}{c}{NA} & \multicolumn{2}{c}{NA} & \multicolumn{2}{c}{NA} \\  
 \midrule
 
\multirow{3}{*}{\textsc{ChemSyn}$\Rightarrow$\textsc{WLP}} 
  & \$700 & 78.81\textsubscript{0.6}\textsuperscript{\textdagger} & (1590) & \textbf{79.80}\textsubscript{0.6}\textsuperscript{\textdagger} & (1590) & 78.97\textsubscript{0.7}\textsuperscript{\textdagger} & (181) & \multicolumn{2}{c}{NA} & \multicolumn{2}{c}{NA} \\ 
 & \$1500 & 79.91\textsubscript{0.4}\textsuperscript{\textdagger} & (3409) & 80.15\textsubscript{0.8}\textsuperscript{\textdagger} & (3409) & \textbf{80.87}\textsubscript{0.7}\textsuperscript{\textdagger} & (2000) & 79.69\textsubscript{0.4}\textsuperscript{\textdagger} & (1590) & 79.44\textsubscript{0.8}\textsuperscript{\textdagger} & (363) \\ 
 & \$2300 & 80.54\textsubscript{0.6}\textsuperscript{\textdagger} & (5227) & 80.97\textsubscript{0.2}\textsuperscript{\textdagger} & (5227) & 81.15\textsubscript{0.6}\textsuperscript{\textdagger} & (3818) & \textbf{81.33}\textsubscript{0.5}\textsuperscript{\textdagger} & (3409) & 80.16\textsubscript{0.7}\textsuperscript{\textdagger} & (2181) \\  \midrule
 
\multirow{3}{*}{\textsc{PubMedM\&M}$\Rightarrow$\textsc{WLP}} 
  & \$700 & 78.34\textsubscript{0.8}\textsuperscript{\textdagger} & (1590) & \textbf{78.44}\textsubscript{1.2}\textsuperscript{\textdagger} & (1590) & 77.98\textsubscript{0.8}\textsuperscript{\textdagger} & (181) & \multicolumn{2}{c}{NA} & \multicolumn{2}{c}{NA} \\ 
 & \$1500 & 79.40\textsubscript{0.6}\textsuperscript{\textdagger} & (3409) & 79.78\textsubscript{0.6}\textsuperscript{\textdagger} & (3409) & \textbf{80.45}\textsubscript{0.2}\textsuperscript{\textdagger} & (2000) & 78.79\textsubscript{1.1}\textsuperscript{\textdagger} & (1590) & 78.76\textsubscript{0.5}\textsuperscript{\textdagger} & (363) \\ 
 & \$2300 & 79.93\textsubscript{0.5}\textsuperscript{\textdagger} & (5227) & 80.04\textsubscript{0.8}\textsuperscript{\textdagger} & (5227) & \textbf{80.85}\textsubscript{0.6}\textsuperscript{\textdagger} & (3818) & 79.49\textsubscript{0.7}\textsuperscript{\textdagger} & (3409) & 80.33\textsubscript{0.3}\textsuperscript{\textdagger} & (2181) \\  
 \bottomrule 
\end{tabular}}
\end{center}
\caption{\label{tab:re_results} Experiment results for Relation Extraction (RE). Similar to the observations in Table \ref{tab:ner_results}, regardless of a small or large budget, prioritizing data annotation in the target domain is the most beneficial. \textsuperscript{\textdagger} indicates results using EasyAdapt (\S \ref{sec:utility_easy}), where source domain data helps. }
\end{table*}

%for a smaller budget (\$700), spending all budget on data annotation and using off-the-shelf language models (\bertbase{} and \bertlarge{}) leads to the best performance, while coupling in-domain pre-training with data annotation is a better combination strategy when a higher budget is available. 



\paragraph{What is the starting budget to consider pre-training an in-domain language model?}
To answer this question, 
we plot development set NER performance for two strategies, \bertbase{} (investing all funds on annotation) and \procbert{} (combining annotation with pre-training), against varying budgets in Figure \ref{fig:budget}. Specifically, the budget of each strategy starts with the pre-training cost of its associated language model, and is increased by 155 USD increments until the total budget reaches the total cost of available data.
%creating the training set for the target domain dataset.
% The budget of each strategy started with the pre-training cost of its associated language model, where only , and we increase it 155 USD each time for data annotation and evaluate model performance until the annotation cost reach the total expense of the training set of the target domain dataset.
% The development set results under two domain adaptation settings \pubmed{}$\Rightarrow$\chemsyn{} and \chemsyn{}$\Rightarrow$\wlp{} are shown in Figure \ref{fig:budget}. 
% For \pubmed{}$\Rightarrow$\chemsyn{}, we can see that \bertbase{} has a clear advantage over \procbert{} when the budget is less than 1000 USD while \procbert{} performs better starting from 1240 USD.
% For both settings, we observe that: 1) Adding a small amount of in-domain labeled data can greatly boost the performance; 2) 
% Like what we find in \S\ref{sec:utility_result}, 
% \bertbase{} (investing all funds on annotation) works better in lower budgets while \procbert{} (combining annotation with pre-training) excels in higher budgets, which further validates our findings in \S\ref{sec:utility_result}.
We observe a similar trend for both \pubmed{}$\Rightarrow$\chemsyn{} and \chemsyn{}$\Rightarrow$\wlp{}: annotation alone works better in lower budgets while in-domain pre-training (\procbert{}) excels at higher budgets.
% , which validates our findings in \S\ref{sec:utility_result}, 
However, the intersection of the curves for these two strategies occurs at different points, which are around 1240 USD and 1705 USD.
%for \pubmed{}$\Rightarrow$\chemsyn{} and \chemsyn{}$\Rightarrow$\wlp{}, respectively.
% the performances of \bertbase{} and \procbert{} intersect at around , but this intersection happens at around for . 
We hypothesize this difference may be because \chemsyn{} is a more constrained domain, requiring less annotated data (\bert{} surpasses 90 F\textsubscript{1} at 155 USD), whereas \wlp{} covers a more diverse range of protocols that include cell cultures, DNA sequencing, etc. 
%\wx{what is the logic of the following sentence?} 
%The later requires more human knowledge to understand the task well, which benefits from prioritizing the data annotation over in-domain pre-training. 
%The main takeaway is that the timing of in-domain pre-training depends on the difficulty of the target task, and the easier the task is, the earlier we should do in-domain pre-training. 

Also note that our estimated annotation cost, $C_a$, (per sentence) includes the annotation of both entity mentions and relations, so our analysis amortizes the cost of pre-training across both tasks.  In a scenario where the NLP practitioner needs to adapt more tasks to the target domain, this could be accounted for simply by dividing the cost of pre-training among tasks, which would shift the black curves in Figure \ref{fig:budget} to the left, making pre-training an economical choice for lower budgets.

%\subsection{Analysis}
%\label{sec:utility_analysis}



% \begin{figure}
% \includegraphics[width=8cm]{figures/chemsyn_ner_budget.pdf}
% \caption{\label{fig:chemsyn_budget} Budget-aware comparison between \bertbase{} and \procbert{} on NER (dev set) for the domain adaptation setting \pubmed{}$\Rightarrow$\chemsyn{}. 
% The budget of each model starts with its pre-training cost, and we evaluate its performance every 155 USD until the annotation cost reaches 4,000 USD, the expense of the \chemsyn{} training set.
% % The annotation cost is increased 155 USD each time until it reaches 4,003 USD, the expense of the \chemsyn{} training set.
% }
% \end{figure}

% \begin{table}[t!]
% \small
% \begin{center}
% % \setlength\tabcolsep{3pt}
% \setlength{\tabcolsep}{3pt}%Tighter
% \scalebox{0.95}{
% \begin{tabular}{lccc}
% \toprule 
% Model (cost) & Seen Entities & Unseen Entities & All \\ \midrule
% \bert{} (\$0)       & \textbf{97.96} & 89.01          & 95.59 \\ 
% \procbert{} (\$620) & 97.57          & \textbf{91.35} & \textbf{95.61} \\ \midrule
% \bert{} (\$0)       & 86.91 & 56.42 & 79.36 \\ 
% \procbert{} (\$620) & \textbf{87.87} & \textbf{59.33} & 79.36 \\
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \caption{\label{tab:anno_pretrain_compare} Comparison (F\textsubscript{1}) between annotation and pre-training.}
% \end{table}

\begin{comment}
\begin{table}[t!]
\small
\begin{center}
\setlength{\tabcolsep}{3pt}%Tighter
\scalebox{1}{
\begin{tabular}{ccc}
% \resizebox{\textwidth}{!}{\begin{tabular}{cccHcccc}
\toprule 
%  & \multicolumn{2}{c}{\pubmed{}$\Rightarrow$\chemsyn{}} & \multicolumn{2}{c}{\chemsyn{}$\Rightarrow$\wlp{}} \\
%  \multirow{2}{*}{\textbf{Category}} & \bertbase{} & \procbert{} \\
%  & \$0 & \$620  \\
\textbf{Category} & \bertbase{} (\$0) & \procbert{} (\$620) \\
% \multirow{4}{c}{\pubmed{}$\Rightarrow$\chemsyn{}} \\
\midrule
\multicolumn{3}{c}{\pubmed{}$\Rightarrow$\chemsyn{}} \\
%  & \pubmed{} & \\
%  & $\Rightarrow$\chemsyn{} & \\
\cmidrule{1-3}
Seen & \textbf{97.96} & 97.57 \\
Unseen & 89.01 & \textbf{91.35} \\
All & 95.59 & \textbf{95.61} \\
\midrule
\multicolumn{3}{c}{\chemsyn{}$\Rightarrow$\wlp{}} \\
%  & \chemsyn{} & \\
%  & $\Rightarrow$\wlp{} & \\
\cmidrule{1-3}
Seen & 86.91 & \textbf{87.87} \\
Unseen & 56.42 & \textbf{59.33} \\
All & 79.36 & 79.36 \\
% \cmidrule(l){2-2}
\bottomrule
\end{tabular}
}
\end{center}
\caption{\label{tab:anno_pretrain_compare} Dev set F\textsubscript{1} score on seen and unseen entities in budget-aware comparison between \bertbase{} and \procbert{} when two models have similar overall performance with two domain adaptation settings. 
% \textbf{Top}: \pubmed{}$\Rightarrow$\chemsyn{}. \textbf{Bottom}: \chemsyn{}$\Rightarrow$\wlp{}. 
\procbert{} has a better performance on unseen entities showing that in-domain pre-training can help improve model's generalization ability.
% NER performance (F\textsubscript{1} score) of \bertbase{} and \procbert{} decomposed by whether
% for two intersections in Figure \ref{fig:budget}.
}
\end{table}
\end{comment}

% \begin{figure}
% \includegraphics[width=8cm]{figures/wlp_ner_budget.pdf}
% \caption{\label{fig:wlp_budget} Budget-aware comparison between \bertbase{} and \procbert{} on NER (dev set) under the domain adaptation setting \chemsyn{}$\Rightarrow$\wlp{}. 
% We also evaluate the performance of each model every 155 USD until the annotation cost reaches 5,050 USD, the expense of the \wlp{} training set.
% % BERT budget ranges from 0 USD to 3875 USD
% % The annotation cost is increased 155 USD each time until it reaches 5,053 USD, the expense of the \wlp{} training set.
% }
% \end{figure}

% \begin{comment}
% In the previous section, we experiment with five different combination strategies under six domain adaptation settings. 
% We show that annotating in-domain data is crucial to domain adaptation especially in low-resource scenarios while spending partial funds on domain-specific pre-training leads to a better performance under higher budgets.  However, there are two important remaining questions: 
% 1) What is the budget threshold that we should start to consider in-domain pre-training when approaching a new domain? 
% 2) Given these two types of domain adaptation methods (\quotes{supervised} data annotation V.S. \quotes{unsupervised} pre-training), what is their difference in adapting to a new domain?
% % how do they impact the target task differently? 
% \end{comment}



% \ar{This paragraph needs to be improved / clarified}
% For the second question, we first searched for the budget where two strategies have the closest performances in Figure \ref{fig:budget}, and then decomposed their performances by whether the gold or predicted entity mentions exist in the training data (seen) or not (unseen). The decomposed results are presented in Table \ref{tab:anno_pretrain_compare}. We can see that \procbert{} has slightly worse performance on "seen" entities and performs much better on "unseen" entities.
% This signals that data annotation can provide more task-specific knowledge while in-domain pre-training can help improve the efficiency of learning task-specific knowledge from limited annotated data.

%\paragraph{When trained under the same budget and achieving similar F\textsubscript{1}, how do \bertbase{} and \procbert{} differ?} 
\paragraph{When using the same budget and achieving similar F\textsubscript{1}, how do pre-training and annotation differ?} In the previous experiments, we show that in-domain pre-training is an effective domain adaptation method especially in high-budget settings. \procbert{} can work very well when trained with less labeled data. %\wx{need to make sure the following sentences are proper English.} 
A plausible explanation is that in-domain pre-training improves generalization to new entities in the target domain, whereas additional annotation improves the performance on entities that are observed in the training corpus.
%, i.e., the model can make correct predictions that are not observed in the training data. 
To evaluate this hypothesis, we compare model predictions of the two strategies at the crossover points in Figure \ref{fig:budget}, and consider each entity in the test set as "Seen" or "Unseen" based on whether it was observed in the training set. Then, we calculate the F\textsubscript{1} score for each category as shown in Table \ref{tab:anno_pretrain_compare}.  Although the models that are compared achieve nearly identical overall performance, the decomposition of performance on seen and unseen entities in Table \ref{tab:anno_pretrain_compare} clearly suggests that in-domain pre-training leads to better generalization on unseen entities, whereas allocating more budget to annotation boosts performance on entities that were seen during training.  This may help provide an explanation for the main finding of this paper: in-domain pre-training results in better generalization on unseen mentions, leading to better marginal utility, but only after enough in-domain annotations are observed to fully cover the head of the distribution.
%We observe that the approach in which most of the budget was expended on pre-training (\procbert{}) performs better on unseen mentions than when the budget is spent entirely on annotation (\bert{}).
%that \procbert{} has a better performance on "Unseen" mentions compared to \bert{} and maintains the overall performance in both domain adaptation settings when trained with less labeled data, validating our generalization hypothesis.


\begin{table}[t!]
\small
\begin{center}
\setlength{\tabcolsep}{5pt}%Tighter
\scalebox{0.95}{
\begin{tabular}{lrcc}
% \resizebox{\textwidth}{!}{\begin{tabular}{cccHcccc}
\toprule 
%  & \multicolumn{2}{c}{\pubmed{}$\Rightarrow$\chemsyn{}} & \multicolumn{2}{c}{\chemsyn{}$\Rightarrow$\wlp{}} \\
% \multirow{2}{*}{\textbf{Source $\Rightarrow$ Target}} & \multirow{2}{*}{\textbf{Entities}} & \bertbase{} & \procbert{} \\
%  & & \$0 & \$620  \\
\textbf{Source} &  \multirow{2}{*}{\textbf{Entities}} & \textbf{\bertbase{}} & \textbf{\procbert{}} \\
\textbf{$\Rightarrow$ Target} & & \$0 & \$620  \\
% \multirow{4}{c}{\pubmed{}$\Rightarrow$\chemsyn{}} \\
\midrule
% \multirow{3}{*}{}
\multirow{1}{*}{\begin{minipage} {.12\textwidth}\vspace{0.3cm} 
\pubmed{} \newline
$\Rightarrow$\chemsyn{} \newline (budget \$1240)\end{minipage}} & seen by both & \textbf{98.29} & 97.71 \\
% \pubmed{}$\Rightarrow$\chemsyn{} & Seen & \textbf{97.96} & 97.57 \\
&  unseen by both & 89.54 & \textbf{91.02} \\
&  seen by BERT & \textbf{95.38} & 94.76 \\
\cmidrule{2-4}
&  All & 95.59 & 95.61 \\
\midrule
\multirow{1}{*}{\begin{minipage} {.12\textwidth}\vspace{0.3cm} 
\chemsyn{} \newline
$\Rightarrow$\wlp{} \newline (budget \$1705) \end{minipage}} & seen by both & \textbf{88.05} & 87.87 \\
% \pubmed{}$\Rightarrow$\chemsyn{} & Seen & \textbf{97.96} & 97.57 \\
&  unseen by both & 56.42 & \textbf{57.08} \\
&  seen by BERT & \textbf{72.72} & 70.79 \\
\cmidrule{2-4}
&  All & 79.36 & 79.36 \\
% \cmidrule(l){2-2}
\bottomrule
\end{tabular}
}
\end{center}
\caption{\label{tab:anno_pretrain_compare} Dev set F\textsubscript{1} on NER for entities seen and unseen in the training data for  \bertbase{} and \procbert{}, when the two achieve very similar overall performance under the same budget constraints. \procbert{} performs better on the unseen entities.}
% showing that in-domain pre-training can help improve model's generalization ability
\end{table}

